Milestones in Autonomous Driving and Intelligent Vehicles Part II: Perception and Planning

Growing interest in autonomous driving (AD) and intelligent vehicles (IVs) is fueled by their promise for enhanced safety, efficiency, and economic benefits. While previous surveys have captured progress in this field, a comprehensive and forward-looking summary is needed. Our work fills this gap through three distinct articles. The first part, a "Survey of Surveys" (SoS), outlines the history, surveys, ethics, and future directions of AD and IV technologies. The second part, "Milestones in Autonomous Driving and Intelligent Vehicles Part I: Control, Computing System Design, Communication, HD Map, Testing, and Human Behaviors" delves into the development of control, computing system, communication, HD map, testing, and human behaviors in IVs. This part, the third part, reviews perception and planning in the context of IVs. Aiming to provide a comprehensive overview of the latest advancements in AD and IVs, this work caters to both newcomers and seasoned researchers. By integrating the SoS and Part I, we offer unique insights and strive to serve as a bridge between past achievements and future possibilities in this dynamic field.

==> body/bib_old.tex <==
%\begin{thebibliography}{1}

\bibliographystyle{IEEEtran}
\bibliography{IEEEabrv,mylib}

%%%survey%%%
publisher={IEEE}
@article{survey_1,
  title={Survey on artificial intelligence for vehicles},
  author={Li, Jun and Cheng, Hong and Guo, Hongliang and Qiu, Shaobo},
  journal={Automotive Innovation},
  volume={1},
  number={1},
  pages={2--14},
  year={2018},
  publisher={Springer}
}

\bibitem{survey_Deep_Multi-modal}
Feng, D., Haase-Schütz, C., Rosenbaum, L., Hertlein, H., Glaeser, C., Timm, F., ... & Dietmayer, K. (2020). Deep multi-modal object detection and semantic segmentation for autonomous driving: Datasets, methods, and challenges. IEEE Transactions on Intelligent Transportation Systems, 22(3), 1341-1360.

%%%dataset%%%
\bibitem{dataset_KITTI}
Geiger, A., Lenz, P., & Urtasun, R. (2012, June). Are we ready for autonomous driving? the kitti vision benchmark suite. In 2012 IEEE conference on computer vision and pattern recognition (pp. 3354-3361). IEEE.

\bibitem{dataset_seg_ADE20K}
Zhou, B., Zhao, H., Puig, X., Xiao, T., Fidler, S., Barriuso, A., & Torralba, A. (2019). Semantic understanding of scenes through the ade20k dataset. International Journal of Computer Vision, 127(3), 302-321.

\bibitem{dataset_seg_VOC}
Everingham, M., Van Gool, L., Williams, C. K., Winn, J., & Zisserman, A. (2010). The pascal visual object classes (voc) challenge. International journal of computer vision, 88(2), 303-338.

\bibitem{dataset_seg_CityScape}
Zhou, B., Zhao, H., Puig, X., Xiao, T., Fidler, S., Barriuso, A., & Torralba, A. (2019). Semantic understanding of scenes through the ade20k dataset. International Journal of Computer Vision, 127(3), 302-321.

\bibitem{dataset_seg_Mapillary_Vistas}
Neuhold, G., Ollmann, T., Rota Bulo, S., & Kontschieder, P. (2017). The mapillary vistas dataset for semantic understanding of street scenes. In Proceedings of the IEEE international conference on computer vision (pp. 4990-4999).

\bibitem{dataset_NYUv2}
Silberman, N., Hoiem, D., Kohli, P., & Fergus, R. (2012, October). Indoor segmentation and support inference from rgbd images. In European conference on computer vision (pp. 746-760). Springer, Berlin, Heidelberg.

%%%localization%%%
\bibitem{loca_1}
Kuutti S ,  Fallah S ,  Katsaros K , et al. A Survey of the State-of-the-Art Localization Techniques and Their Potentials for Autonomous Vehicle Applications[J]. IEEE Internet of Things Journal, 2018:829-846.

\bibitem{loca_2}
Liang L ,  Ming Y ,  Bing W , et al. An overview on sensor map based localization for automated driving[C]// Urban Remote Sensing Event. IEEE, 2017.

\bibitem{loca_3}
Wang Y ,  Zhang W . A Survey of Simultaneous Localization and Mapping on Unstructured Lunar Complex Environment[J]. Journal of Zhengzhou University(Engineering Science), 2018.

\bibitem{loca_4}
Luo Q , Y Cao, Liu J , et al. Localization and Navigation in Autonomous Driving: Threats and Countermeasures[J]. IEEE Wireless Communications, 2019, 26(4):38-45.

\bibitem{loca_5}
Debeunne C ,  Vivet D . A Review of Visual-LiDAR Fusion based Simultaneous Localization and Mapping[J]. Sensors, 2020, 20(7):2068.

\bibitem{loca_6}
Singandhupe A ,  La H M . A Review of SLAM Techniques and Security in Autonomous Driving[C] 2019 Third IEEE International Conference on Robotic Computing (IRC). IEEE, 2019.

\bibitem{loca_7}
Takleh T ,  Bakar N A ,  Rahman S A , et al. A Brief Survey on SLAM Methods in Autonomous Vehicle[J]. International Journal of Engineering & Technology, 2018, 7(4):38-43.

\bibitem{loca_8}
Gao B ,  Lang H ,  Ren J . Stereo Visual SLAM for Autonomous Vehicles: A Review[C]// 2020 IEEE International Conference on Systems, Man, and Cybernetics (SMC). IEEE, 2020.

\bibitem{loca_9}
Wong K ,  Gu Y ,  Kamijo S . Mapping for Autonomous Driving: Opportunities and Challenges[J]. IEEE Intelligent Transportation Systems Magazine, 2020, PP(99).

\bibitem{loca_10}
Jonnavithula N ,  Lyu Y ,  Zhang Z . LiDAR Odometry Methodologies for Autonomous Driving: A Survey[J].  2021.

\bibitem{loca_11}
Guo H ,  D  Cao,  Hong C , et al. Vehicle dynamic state estimation: state of the art schemes and perspectives[J]. IEEE/CAA Journal of Automatica Sinica, 2018, 5(002):418-431.

\bibitem{loca_12}
Chehri A ,  Quadar N ,  Saadane R . Survey on localization methods for autonomous vehicles in smart cities[C]// the 4th International Conference. 2019.

\bibitem{loca_14}
Leurent E . A Survey of State-Action Representations for Autonomous Driving. 

\bibitem{loca_15}
Chen S ,  Liu B ,  Feng C , et al. 3D Point Cloud Processing and Learning for Autonomous Driving: Impacting Map Creation, Localization, and Perception[J]. IEEE Signal Processing Magazine, 2021, 38(1):68-86.

\bibitem{loca_16}
G. Bresson, Z. Alsayed, L. Yu and S. Glaser,” Simultaneous Localization and Mapping: A Survey of Current Trends in Autonomous Driving,” IEEE Transactions on Intelligent Vehicles,pp. 194-220, 2017.

\bibitem{loca_17}C. Gentner, T. Jost, W. Wang, S. Zhang, A. Dammann and U.C.Fiebig,” Multipath Assisted Positioning with Simultaneous Localization and Mapping,” IEEE Transactions on Wireless Communications, pp. 1536-1276, 2016.

\bibitem{loca_18}
K.-H. Jo and J. Lee, "Multi-robot cooperative localization with optimally fused information of odometer and gps," in International Conference on Control, Automation and Systems 2007, 2007.

\bibitem{loca_19}
C. Cadena, L. Carlone, H. Carrillo, Y. Latif, D. Scaramuzza, J. Neira,I. Reid, and J. J. Leonard. Past, present, and future of simultaneous localization and mapping: Toward the robust-perception age. IEEETrans. on Robotics, 32(6):1309–1332, Dec 2016.

\bibitem{loca_20}
Frank Steinbrücker, Jürgen Sturm, and Daniel Cremers. Real-time visual odometry from dense rgb-d images. In 2011 IEEE International Conference on Computer Vision Workshops (ICCV Workshops), pages719–722. IEEE, 2011.

\bibitem{loca_21}
Christian Kerl, Jürgen Sturm, and Daniel Cremers. Robust odometry estimation for rgb-d cameras. In 2013 IEEE International Conferenceon Robotics and Automation, pages 3748–3754. IEEE, 2013.

\bibitem{loca_22}
Newcombe, R.A.; Lovegrove, S.J.; Davison, A.J. DTAM: Dense tracking and mapping in real-time.In Proceedings of the 2011 International Conference on Computer Vision, Barcelona, Spain, 6–13 November 2011; pp. 2320–2327.

\bibitem{loca_23}
Engel, J.; Schöps, T.; Cremers, D. LSD-SLAM: Large-scale direct monocular SLAM. In Proceedings of theEuropean Conference on Computer Vision, Zurich, Switzerland, 6–12 September 2014; pp. 834–849.

\bibitem{loca_24}
Forster, C.; Pizzoli, M.; Scaramuzza, D. SVO: Fast semi-direct monocular visual odometry. In Proceedings of the 2014 IEEE International Conference on Robotics and Automation (ICRA), Hong Kong, China,31 May–7 June 2014; pp. 15–22.

\bibitem{loca_25}
Engel, J.; Koltun, V.; Cremers, D. Direct sparse odometry. IEEE Trans. Pattern Anal. Mach. Intell. 2017,40, 611–625. [CrossRef]

\bibitem{loca_26}
Wang, R.; Schworer, M.; Cremers, D. Stereo DSO: Large-scale direct sparse visual odometry withstereo cameras. In Proceedings of the IEEE International Conference on Computer Vision, Venice, Italy,22–29 October 2017; pp. 3903–3911.

\bibitem{loca_27}
E. Eade and T. Drummond, “Scalable Monocular SLAM,” in IEEE Computer Society Conference on Computer Vision and Pattern Recognition, vol. 1, 2006, pp. 469–476.

\bibitem{loca_28}
D. Chetverikov, D. Svirko, D. Stepanov, and P. Krsek, “The trimmed iterative closest point algorithm,” in Object recognition supported by user interaction for service robots, vol. 3. IEEE, 2002, pp. 545–548.

\bibitem{loca_29}
A. Segal, D. Haehnel, and S. Thrun, “Generalized-icp.” in Robotics: science and systems, vol. 2, no. 4. Seattle, WA, 2009, p. 435. 

\bibitem{loca_30}
S. Bouaziz, A. Tagliasacchi, and M. Pauly, “Sparse iterative closest point,” in Computer graphics forum, vol. 32, no. 5. Wiley Online Library, 2013, pp. 113–123. 

\bibitem{loca_31}
A. L. Pavlov, G. W. Ovchinnikov, D. Y. Derbyshev, D. Tsetserukou, and I. V. Oseledets, “Aa-icp: Iterative closest point with anderson acceleration,” in 2018 IEEE International Conference on Robotics and Automation (ICRA). IEEE, 2018, pp. 3407–3412. 

\bibitem{loca_32}
S. A. Parkison, L. Gan, M. G. Jadidi, and R. M. Eustice, “Semantic iterative closest point through expectation-maximization.” in BMVC, 2018, p. 280.

\bibitem{loca_33}
C. Choy, W. Dong, and V. Koltun, “Deep global registration,” in Proceedings of the IEEE/CVF conference on computer vision and pattern recognition, 2020, pp. 2514–2523.

\bibitem{loca_34}
X. Chen, A. Milioto, E. Palazzolo, P. Giguere, J. Behley, and C. Stachniss, “Suma++: Efficient lidar-based semantic slam,” in 2019 IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS). IEEE, 2019, pp. 4530–4537.

\bibitem{loca_35}
X. Zheng and J. Zhu, “Efficient lidar odometry for autonomous driving,” arXiv preprint arXiv:2104.10879, 2021.

\bibitem{loca_36}
J. Zhang and S. Singh, “Loam: Lidar odometry and mapping in realtime.” in Robotics: Science and Systems, vol. 2, no. 9, 2014.

\bibitem{loca_37}
T. Shan and B. Englot, “Lego-loam: Lightweight and groundoptimized lidar odometry and mapping on variable terrain,” in 2018 IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS). IEEE, 2018, pp. 4758–4765

\bibitem{loca_38}
Q. M. Thomas, O. Wasenmuller, and D. Stricker, “Delio: Decoupled ¨ lidar odometry,” in 2019 IEEE Intelligent Vehicles Symposium (IV). IEEE, 2019, pp. 1549–1556.

\bibitem{loca_39}
S. Lee, C. Kim, S. Cho, S. Myoungho, and K. Jo, “Robust 3- dimension point cloud mapping in dynamic environment using pointwise static probability-based ndt scan-matching,” IEEE Access, vol. 8, pp. 175 563–175 575, 2020.

\bibitem{loca_40}
Shan T ,  Englot B ,  Ratti C , et al. LVI-SAM: Tightly-coupled Lidar-Visual-Inertial Odometry via Smoothing and Mapping[J].  2021.

\bibitem{loca_41}
Lin J ,  Zheng C ,  Xu W , et al. R2LIVE: A Robust, Real-time, LiDAR-Inertial-Visual tightly-coupled state Estimator and mapping[J].  2021.

\bibitem{loca_42}
Tong, Qin, Peiliang, et al. VINS-Mono: A Robust and Versatile Monocular Visual-Inertial State Estimator[J]. IEEE Transactions on Robotics, 2018.

\bibitem{loca_43}
Hao L ,  Li H ,  Zhang Q , et al. LMVI-SLAM: Robust Low-Light Monocular Visual-Inertial Simultaneous Localization and Mapping[C]// 2019 IEEE International Conference on Robotics and Biomimetics (ROBIO). IEEE, 2019.

\bibitem{loca_44}
Zuo X ,  Geneva P ,  Lee W , et al. LIC-Fusion: LiDAR-Inertial-Camera Odometry[J]. IROS, 2019.

\bibitem{loca_45}
S. W. Chen, G. V. Nardari, E. S. Lee, C. Qu, X. Liu, R. A. F. Romero, and V. Kumar, “Sloam: Semantic lidar odometry and mapping for forest inventory,” IEEE Robotics and Automation Letters, vol. 5, no. 2, pp. 612–619, 2020.

\bibitem{loca_46}
Elhousni M ,  Huang X . A Survey on 3D LiDAR Localization for Autonomous Vehicles[C]// 2020 IEEE Intelligent Vehicles Symposium (IV). IEEE, 2020.

\bibitem{loca_47}
C. Cadena, L. Carlone, H. Carillo, Y. Latif, D. Scaramuzza, J.Neira, I. Reid and J. J. Leonard,” Past, Present and Future of Samultaneous Localization and Mapping: Toward the Robust Perception Age,” IEEE Transactions on Robotics, pp. 1309-1332, 2016. 

\bibitem{loca_48}
X. Xie, Y. Yu, X. Lin and C. Sun,” An EKF SLAM Algorithm for Mobile Robot with Sensor Bias Estimation,” 32nd Youth Academic Annual Conference of Chinese Association of Automation (YAC),pp. 281-285, 2017. 

\bibitem{loca_49}
S. Thrun and J. J. Leonard, “Simultaneous localization and mapping,” in Springer Handbook of Robotics. New York, NY, USA: Springer -Verlag, 2008, pp. 871 –889.

\bibitem{loca_50}
Sun F, Zhou Y, Li C, et al. Research on active SLAM with fusion of monocular vision and laser range data[C]. Jinan: In IEEE World Congress on Intelligent Control and Automation, 2010: 6550–6554.

\bibitem{loca_51}
Arandjelovic R, Gronat P, Torll A, et al. NetVLAD: CNN architecture for weakly supervised place recognition[C]. New York: In Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition, 2016: 5297-5307

\bibitem{loca_52}
én M, García S, Barea R, et al. A Multi-Sensorial Simultaneous Localization and Mapping (SLAM) System for Low-Cost Micro Aerial Vehicles in GPS-Denied Environments[J]. Sensors, 2017, 17(4): 802-829

\bibitem{loca_53}
Graeter J, Wilczynski A, Lauer M. Limo: Lidar-monocular visual odometry[C]. In IEEE/RSJ International Conference on Intelligent Robots and Systems. Madrid, Spain, 2018: 7872–7879

\bibitem{loca_54}
Shin Y S, Park Y S, Kim A. Direct visual SLAM using sparse depth for camera-lidar system[C]. Australia: In IEEE International Conference on Robotics and Automation Brisbane, 2018: 1–8.

\bibitem{loca_55}
De Silva V, Roche J, Kondoz A. Fusion of LiDAR and camera sensor data for environment sensing in driverless vehicles[J]. arXiv2018, arXiv: 1710.06230.

\bibitem{loca_56}
M. Magnusson, ‘‘The three-dimensional normal-distributions transform—An efficient representation for registration, surface analysis, and loop detection,’’ Ph.D. dissertation, Graduate School Robot. Automat. Process Control, Örebro Univ., Örebro, Sweden, 2009

\bibitem{loca_57}
M. Magnusson, A. Nuchter, C. Lorken, A. J. Lilienthal, and J. Hertzberg,‘‘Evaluation of 3D registration reliability and speed—A comparison of ICP and NDT,’’ in Proc. IEEE Int. Conf. Robot. Autom., May 2009,pp. 3907–3912.

\bibitem{loca_58}
‘‘A 3-D scan matching using improved 3-D normal distributions transform for mobile robotic mapping,’’ in Proc. IEEE/RSJ Int. Conf. Intell. Robots Syst., Oct. 2006, pp. 3068–3073.

%%%perception_scene%%%

\bibitem{scene_FCN}
Long, J., Shelhamer, E., & Darrell, T. (2015). Fully convolutional networks for semantic segmentation. In Proceedings of the IEEE conference on computer vision and pattern recognition (pp. 3431-3440).

\bibitem{scene_segnet}
Badrinarayanan, V., Kendall, A., & Cipolla, R. (2017). Segnet: A deep convolutional encoder-decoder architecture for image segmentation. IEEE transactions on pattern analysis and machine intelligence, 39(12), 2481-2495.

\bibitem{scene_dilated}
Yu, F., & Koltun, V. (2015). Multi-scale context aggregation by dilated convolutions. arXiv preprint arXiv:1511.07122.

\bibitem{scene_DeepLabv1}
Chen, L. C., Papandreou, G., Kokkinos, I., Murphy, K., & Yuille, A. L. (2014). Semantic image segmentation with deep convolutional nets and fully connected crfs. arXiv preprint arXiv:1412.7062.

\bibitem{scene_DeepLabv2}
Chen, L. C., Papandreou, G., Kokkinos, I., Murphy, K., & Yuille, A. L. (2017). Deeplab: Semantic image segmentation with deep convolutional nets, atrous convolution, and fully connected crfs. IEEE transactions on pattern analysis and machine intelligence, 40(4), 834-848.

\bibitem{scene_RefineNet}
Lin, G., Milan, A., Shen, C., & Reid, I. (2017). Refinenet: Multi-path refinement networks for high-resolution semantic segmentation. In Proceedings of the IEEE conference on computer vision and pattern recognition (pp. 1925-1934).

\bibitem{scene_PSP}
Zhao, H., Shi, J., Qi, X., Wang, X., & Jia, J. (2017). Pyramid scene parsing network. In Proceedings of the IEEE conference on computer vision and pattern recognition (pp. 2881-2890).

\bibitem{scene_DeepLabv3}
Chen, L. C., Papandreou, G., Schroff, F., & Adam, H. (2017). Rethinking atrous convolution for semantic image segmentation. arXiv preprint arXiv:1706.05587.

\bibitem{scene_Unet}
Ronneberger, O., Fischer, P., & Brox, T. (2015, October). U-net: Convolutional networks for biomedical image segmentation. In International Conference on Medical image computing and computer-assisted intervention (pp. 234-241). Springer, Cham.

\bibitem{scene_Unet}
Ronneberger, O., Fischer, P., & Brox, T. (2015, October). U-net: Convolutional networks for biomedical image segmentation. In International Conference on Medical image computing and computer-assisted intervention (pp. 234-241). Springer, Cham.

\bibitem{scene_Unet++}
Zhou, Z., Rahman Siddiquee, M. M., Tajbakhsh, N., & Liang, J. (2018). Unet++: A nested u-net architecture for medical image segmentation. In Deep learning in medical image analysis and multimodal learning for clinical decision support (pp. 3-11). Springer, Cham.

\bibitem{scene_OCRNet}
Yuan, Y., Chen, X., & Wang, J. (2020, August). Object-contextual representations for semantic segmentation. In European conference on computer vision (pp. 173-190). Springer, Cham.

\bibitem{scene_OCNet}
Yuan, Y., Huang, L., Guo, J., Zhang, C., Chen, X., & Wang, J. (2018). Ocnet: Object context network for scene parsing. arXiv preprint arXiv:1809.00916.

\bibitem{scene_multi_scale_attention}
Tao, A., Sapra, K., & Catanzaro, B. (2020). Hierarchical multi-scale attention for semantic segmentation. arXiv preprint arXiv:2005.10821.

\bibitem{scene_boundary_aware_segmentation}
Borse, S., Wang, Y., Zhang, Y., & Porikli, F. (2021). Inverseform: A loss function for structured boundary-aware segmentation. In Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (pp. 5901-5911).

\bibitem{scene_intrinsic_relevance}
Cai, Y., Dai, L., Wang, H., & Li, Z. (2021). Multi-target pan-class intrinsic relevance driven model for improving semantic segmentation in autonomous driving. IEEE Transactions on Image Processing, 30, 9069-9084.

\bibitem{scene_Naive_student}
Chen, L. C., Lopes, R. G., Cheng, B., Collins, M. D., Cubuk, E. D., Zoph, B., ... & Shlens, J. (2020, August). Naive-student: Leveraging semi-supervised learning in video sequences for urban scene segmentation. In European Conference on Computer Vision (pp. 695-714). Springer, Cham.

\bibitem{scene_unsupervised_domain}
Erkent, Ö., & Laugier, C. (2020). Semantic segmentation with unsupervised domain adaptation under varying weather conditions for autonomous vehicles. IEEE Robotics and Automation Letters, 5(2), 3580-3587.

\bibitem{scene_Warp_Refine_Propagation}
Ganeshan, A., Vallet, A., Kudo, Y., Maeda, S. I., Kerola, T., Ambrus, R., ... & Gaidon, A. (2021). Warp-Refine Propagation: Semi-Supervised Auto-labeling via Cycle-consistency. In Proceedings of the IEEE/CVF International Conference on Computer Vision (pp. 15499-15509).

\bibitem{scene_Mask_RCNN}
He, K., Gkioxari, G., Dollár, P., & Girshick, R. (2017). Mask r-cnn. In Proceedings of the IEEE international conference on computer vision (pp. 2961-2969).

\bibitem{scene_HTC}
Chen, K., Pang, J., Wang, J., Xiong, Y., Li, X., Sun, S., ... & Lin, D. (2019). Hybrid task cascade for instance segmentation. In Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (pp. 4974-4983).

\bibitem{scene_Explicit}
Xu, W., Wang, H., Qi, F., & Lu, C. (2019). Explicit shape encoding for real-time instance segmentation. In Proceedings of the IEEE/CVF International Conference on Computer Vision (pp. 5168-5177).

\bibitem{scene_Yolact}
Bolya, D., Zhou, C., Xiao, F., & Lee, Y. J. (2019). Yolact: Real-time instance segmentation. In Proceedings of the IEEE/CVF international conference on computer vision (pp. 9157-9166).

\bibitem{scene_Blendmask}
Chen, H., Sun, K., Tian, Z., Shen, C., Huang, Y., & Yan, Y. (2020). Blendmask: Top-down meets bottom-up for instance segmentation. In Proceedings of the IEEE/CVF conference on computer vision and pattern recognition (pp. 8573-8581).

\bibitem{scene_Centermask}
Lee, Y., & Park, J. (2020). Centermask: Real-time anchor-free instance segmentation. In Proceedings of the IEEE/CVF conference on computer vision and pattern recognition (pp. 13906-13915).

\bibitem{scene_Embedmask}
Ying, H., Huang, Z., Liu, S., Shao, T., & Zhou, K. (2019). Embedmask: Embedding coupling for one-stage instance segmentation. arXiv preprint arXiv:1912.01954.

\bibitem{scene_Mask_encoding}
Zhang, R., Tian, Z., Shen, C., You, M., & Yan, Y. (2020). Mask encoding for single shot instance segmentation. In Proceedings of the IEEE/CVF conference on computer vision and pattern recognition (pp. 10226-10235).

\bibitem{scene_Conditional}
Tian, Z., Shen, C., & Chen, H. (2020, August). Conditional convolutions for instance segmentation. In European conference on computer vision (pp. 282-298). Springer, Cham.

\bibitem{scene_Solov2}
Wang, X., Zhang, R., Kong, T., Li, L., & Shen, C. (2020). Solov2: Dynamic and fast instance segmentation. Advances in Neural information processing systems, 33, 17721-17732.

\bibitem{scene_Ssap}
Gao, N., Shan, Y., Wang, Y., Zhao, X., Yu, Y., Yang, M., & Huang, K. (2019). Ssap: Single-shot instance segmentation with affinity pyramid. In Proceedings of the IEEE/CVF International Conference on Computer Vision (pp. 642-651).

\bibitem{scene_Polytransform}
Liang, J., Homayounfar, N., Ma, W. C., Xiong, Y., Hu, R., & Urtasun, R. (2020). Polytransform: Deep polygon transformer for instance segmentation. In Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (pp. 9131-9140).

\bibitem{scene_Look_closer_to_segment_better}
Tang, C., Chen, H., Li, X., Li, J., Zhang, Z., & Hu, X. (2021). Look closer to segment better: Boundary patch refinement for instance segmentation. In Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (pp. 13926-13935).

\bibitem{scene_Scaling_wide}
Chen, L. C., Wang, H., & Qiao, S. (2020). Scaling wide residual networks for panoptic segmentation. arXiv preprint arXiv:2011.11675.

\bibitem{scene_Panoptic_segmentation}
Kirillov, A., He, K., Girshick, R., Rother, C., & Dollár, P. (2019). Panoptic segmentation. In Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (pp. 9404-9413).

\bibitem{scene_Panoptic_segmentation_joint}
De Geus, D., Meletis, P., & Dubbelman, G. (2018). Panoptic segmentation with a joint semantic and instance segmentation network. arXiv preprint arXiv:1809.02110.

\bibitem{scene_Panoptic_FPN}
Kirillov, A., Girshick, R., He, K., & Dollár, P. (2019). Panoptic feature pyramid networks. In Proceedings of the IEEE/CVF conference on computer vision and pattern recognition (pp. 6399-6408).

\bibitem{scene_AUNet}
Li, Y., Chen, X., Zhu, Z., Xie, L., Huang, G., Du, D., & Wang, X. (2019). Attention-guided unified network for panoptic segmentation. In Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (pp. 7026-7035).

\bibitem{scene_UPNet}
Xiong, Y., Liao, R., Zhao, H., Hu, R., Bai, M., Yumer, E., & Urtasun, R. (2019). Upsnet: A unified panoptic segmentation network. In Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (pp. 8818-8826).

\bibitem{scene_Panoptic_FCN}
Li, Y., Zhao, H., Qi, X., Wang, L., Li, Z., Sun, J., & Jia, J. (2021). Fully convolutional networks for panoptic segmentation. In Proceedings of the IEEE/CVF conference on computer vision and pattern recognition (pp. 214-223).

\bibitem{scene_Panoptic_SegFormer}
Li, Z., Wang, W., Xie, E., Yu, Z., Anandkumar, A., Alvarez, J. M., ... & Lu, T. (2022). Panoptic SegFormer: Delving deeper into panoptic segmentation with transformers. In Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (pp. 1280-1289).

\bibitem{scene_Improving_panoptic_segmentation}
Porzi, L., Bulo, S. R., & Kontschieder, P. (2021). Improving panoptic segmentation at all scales. In Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (pp. 7302-7311).

\bibitem{scene_TASC}
Li, J., Raventos, A., Bhargava, A., Tagawa, T., & Gaidon, A. (2018). Learning to fuse things and stuff. arXiv preprint arXiv:1812.01192.

\bibitem{scene_Axial_deeplab}
Wang, H., Zhu, Y., Green, B., Adam, H., Yuille, A., & Chen, L. C. (2020, August). Axial-deeplab: Stand-alone axial-attention for panoptic segmentation. In European Conference on Computer Vision (pp. 108-126). Springer, Cham.

\bibitem{scene_Depth_completion}
Uhrig, J., Schneider, N., Schneider, L., Franke, U., Brox, T., & Geiger, A. (2017, October). Sparsity invariant cnns. In 2017 international conference on 3D Vision (3DV) (pp. 11-20). IEEE.

\bibitem{scene_Sparse_and_dense_data_with_cnns}
Jaritz, M., De Charette, R., Wirbel, E., Perrotton, X., & Nashashibi, F. (2018, September). Sparse and dense data with cnns: Depth completion and semantic segmentation. In 2018 International Conference on 3D Vision (3DV) (pp. 52-60). IEEE.

\bibitem{scene_Hms_net}
Huang, Z., Fan, J., Cheng, S., Yi, S., Wang, X., & Li, H. (2019). Hms-net: Hierarchical multi-scale sparsity-invariant network for sparse depth completion. IEEE Transactions on Image Processing, 29, 3429-3441.

\bibitem{scene_Uncertainty_aware_cnns}
Eldesokey, A., Felsberg, M., Holmquist, K., & Persson, M. (2020). Uncertainty-aware cnns for depth completion: Uncertainty from beginning to end. In Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (pp. 12014-12023).

\bibitem{scene_Dfinenet}
Zhang, Y., Nguyen, T., Miller, I. D., Shivakumar, S. S., Chen, S., Taylor, C. J., & Kumar, V. (2019). Dfinenet: Ego-motion estimation and depth refinement from sparse, noisy depth input with rgb guidance. arXiv preprint arXiv:1903.06397.

\bibitem{scene_From_depth_what_can_you_see}
Lu, K., Barnes, N., Anwar, S., & Zheng, L. (2020). From depth what can you see? Depth completion via auxiliary image reconstruction. In Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (pp. 11306-11315).

\bibitem{scene_Confidence_propagation}
Eldesokey, A., Felsberg, M., & Khan, F. S. (2019). Confidence propagation through cnns for guided sparse depth regression. IEEE transactions on pattern analysis and machine intelligence, 42(10), 2423-2436.

\bibitem{scene_Uncertainty_driven_loss}
Zhu, Y., Dong, W., Li, L., Wu, J., Li, X., & Shi, G. (2021). Robust depth completion with uncertainty-driven loss functions. arXiv preprint arXiv:2112.07895.

\bibitem{scene_Depth_normal_constraints}
Xu, Y., Zhu, X., Shi, J., Zhang, G., Bao, H., & Li, H. (2019). Depth completion from sparse lidar data with depth-normal constraints. In Proceedings of the IEEE/CVF International Conference on Computer Vision (pp. 2811-2820).

\bibitem{scene_Self_supervised_sparse_to_dense}
Ma, F., Cavalheiro, G. V., & Karaman, S. (2019, May). Self-supervised sparse-to-dense: Self-supervised depth completion from lidar and monocular camera. In 2019 International Conference on Robotics and Automation (ICRA) (pp. 3288-3295). IEEE.

\bibitem{scene_Geometry_Aware_Embedding}
Du, W., Chen, H., Yang, H., & Zhang, Y. (2022). Depth Completion using Geometry-Aware Embedding. arXiv preprint arXiv:2203.10912.

\bibitem{scene_Joint_2d_3d}
Chen, Y., Yang, B., Liang, M., & Urtasun, R. (2019). Learning joint 2d-3d representations for depth completion. In Proceedings of the IEEE/CVF International Conference on Computer Vision (pp. 10023-10032).

\bibitem{scene_Adaptive_context_aware}
Zhao, S., Gong, M., Fu, H., & Tao, D. (2021). Adaptive context-aware multi-modal network for depth completion. IEEE Transactions on Image Processing, 30, 5264-5276.

\bibitem{scene_Penet}
Hu, M., Wang, S., Li, B., Ning, S., Fan, L., & Gong, X. (2021, May). Penet: Towards precise and efficient image guided depth completion. In 2021 IEEE International Conference on Robotics and Automation (ICRA) (pp. 13656-13662). IEEE.

\bibitem{scene_Learning_guided}
Tang, J., Tian, F. P., Feng, W., Li, J., & Tan, P. (2020). Learning guided convolutional network for depth completion. IEEE Transactions on Image Processing, 30, 1116-1129.

\bibitem{scene_RigNet}
Yan, Z., Wang, K., Li, X., Zhang, Z., Xu, B., Li, J., & Yang, J. (2021). RigNet: Repetitive image guided network for depth completion. arXiv preprint arXiv:2107.13802.

\bibitem{scene_SemAttNet}
Nazir, D., Liwicki, M., Stricker, D., & Afzal, M. Z. (2022). SemAttNet: Towards Attention-based Semantic Aware Guided Depth Completion. arXiv preprint arXiv:2204.13635.

\bibitem{scene_Dynamic_spatial_propagation}
Lin, Y., Cheng, T., Zhong, Q., Zhou, W., & Yang, H. (2022). Dynamic spatial propagation network for depth completion. arXiv preprint arXiv:2202.09769.

%%% scene_depth_estimation%%%
\bibitem{scene_Deepstereo}
lynn, J., Neulander, I., Philbin, J., & Snavely, N. (2016). Deepstereo: Learning to predict new views from the world's imagery. In Proceedings of the IEEE conference on computer vision and pattern recognition (pp. 5515-5524).

\bibitem{scene_NASD}
Kusupati, U., Cheng, S., Chen, R., & Su, H. (2020). Normal assisted stereo depth estimation. In Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (pp. 2189-2199).

\bibitem{scene_Indoor_scene_structure_analysis}
Zhuo, W., Salzmann, M., He, X., & Liu, M. (2015). Indoor scene structure analysis for single image depth estimation. In Proceedings of the IEEE Conference on Computer Vision and Pattern recognition (pp. 614-622).

\bibitem{scene_Depth_map_prediction}
Eigen, D., Puhrsch, C., & Fergus, R. (2014). Depth map prediction from a single image using a multi-scale deep network. Advances in neural information processing systems, 27.

\bibitem{scene_Semi_supervised_deep_learning}
Kuznietsov, Y., Stuckler, J., & Leibe, B. (2017). Semi-supervised deep learning for monocular depth map prediction. In Proceedings of the IEEE conference on computer vision and pattern recognition (pp. 6647-6655).

\bibitem{scene_Unsupervised_cnn}
Garg, R., Bg, V. K., Carneiro, G., & Reid, I. (2016, October). Unsupervised cnn for single view depth estimation: Geometry to the rescue. In European conference on computer vision (pp. 740-756). Springer, Cham.

\bibitem{scene_Refinedmpl}
Vianney, J. M. U., Aich, S., & Liu, B. (2019). Refinedmpl: Refined monocular pseudolidar for 3d object detection in autonomous driving. arXiv preprint arXiv:1911.09712.

\bibitem{scene_Multi_scale_continuous_crfs}
Xu, D., Ricci, E., Ouyang, W., Wang, X., & Sebe, N. (2017). Multi-scale continuous crfs as sequential deep networks for monocular depth estimation. In Proceedings of the IEEE conference on computer vision and pattern recognition (pp. 5354-5362).

\bibitem{scene_Pad_Net}
Xu, D., Ouyang, W., Wang, X., & Sebe, N. (2018). Pad-net: Multi-tasks guided prediction-and-distillation network for simultaneous depth estimation and scene parsing. In Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition (pp. 675-684).

\bibitem{scene_Transformer_based_attention}
Yang, G., Tang, H., Ding, M., Sebe, N., & Ricci, E. (2021). Transformer-based attention networks for continuous pixel-wise prediction. In Proceedings of the IEEE/CVF International Conference on Computer Vision (pp. 16269-16279).

\bibitem{scene_P3Depth}
Patil, V., Sakaridis, C., Liniger, A., & Van Gool, L. (2022). P3Depth: Monocular Depth Estimation with a Piecewise Planarity Prior. In Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (pp. 1610-1621).

\bibitem{scene_DORN}
Fu, H., Gong, M., Wang, C., Batmanghelich, K., & Tao, D. (2018). Deep ordinal regression network for monocular depth estimation. In Proceedings of the IEEE conference on computer vision and pattern recognition (pp. 2002-2011).

\bibitem{scene_Multidepth}
Liebel, L., & Körner, M. (2019, October). Multidepth: Single-image depth estimation via multi-task regression and classification. In 2019 IEEE Intelligent Transportation Systems Conference (ITSC) (pp. 1440-1447). IEEE.

\bibitem{scene_HGR}
Zhang, Z., Xu, C., Yang, J., Tai, Y., & Chen, L. (2018). Deep hierarchical guidance and regularization learning for end-to-end depth estimation. Pattern Recognition, 83, 430-442.

\bibitem{scene_SDNet}
Ochs, M., Kretz, A., & Mester, R. (2019, September). SDNet: Semantically guided depth estimation network. In German conference on pattern recognition (pp. 288-302). Springer, Cham.

\bibitem{scene_Pattern_affinitive_propagation_across_depth}
Zhang, Z., Cui, Z., Xu, C., Yan, Y., Sebe, N., & Yang, J. (2019). Pattern-affinitive propagation across depth, surface normal and semantic segmentation. In Proceedings of the IEEE/CVF conference on computer vision and pattern recognition (pp. 4106-4115).

\bibitem{scene_From_big_to_small}
Lee, J. H., Han, M. K., Ko, D. W., & Suh, I. H. (2019). From big to small: Multi-scale local planar guidance for monocular depth estimation. arXiv preprint arXiv:1907.10326.

\bibitem{scene_Enforcing_geometric_constraints}
Yin, W., Liu, Y., Shen, C., & Yan, Y. (2019). Enforcing geometric constraints of virtual normal for depth prediction. In Proceedings of the IEEE/CVF International Conference on Computer Vision (pp. 5684-5693).

\bibitem{scene_BANet}
Aich, S., Vianney, J. M. U., Islam, M. A., & Liu, M. K. B. (2021, May). Bidirectional attention network for monocular depth estimation. In 2021 IEEE International Conference on Robotics and Automation (ICRA) (pp. 11746-11752). IEEE.

\bibitem{scene_3D_packing}
Guizilini, V., Ambrus, R., Pillai, S., Raventos, A., & Gaidon, A. (2020). 3d packing for self-supervised monocular depth estimation. In Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (pp. 2485-2494).

\bibitem{scene_monodepth2}
Godard, C., Mac Aodha, O., Firman, M., & Brostow, G. J. (2019). Digging into self-supervised monocular depth estimation. In Proceedings of the IEEE/CVF International Conference on Computer Vision (pp. 3828-3838).

\bibitem{scene_Gcndepth}
Masoumian, A., Rashwan, H. A., Abdulwahab, S., Cristiano, J., & Puig, D. (2021). Gcndepth: Self-supervised monocular depth estimation based on graph convolutional network. arXiv preprint arXiv:2112.06782.

\bibitem{scene_Unsupervised_monocular_depth_estimation}
Godard, C., Mac Aodha, O., & Brostow, G. J. (2017). Unsupervised monocular depth estimation with left-right consistency. In Proceedings of the IEEE conference on computer vision and pattern recognition (pp. 270-279).

\bibitem{scene_Self_supervised_monocular_depth_estimation}
Klingner, M., Termöhlen, J. A., Mikolajczyk, J., & Fingscheidt, T. (2020, August). Self-supervised monocular depth estimation: Solving the dynamic object problem by semantic guidance. In European Conference on Computer Vision (pp. 582-600). Springer, Cham.

\bibitem{scene_Dipe}
Jiang, H., Ding, L., Sun, Z., & Huang, R. (2020, October). Dipe: Deeper into photometric errors for unsupervised learning of depth and ego-motion from monocular videos. In 2020 IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS) (pp. 10061-10067). IEEE.

\bibitem{scene_MLDA_Net}
Song, X., Li, W., Zhou, D., Dai, Y., Fang, J., Li, H., & Zhang, L. (2021). MLDA-Net: Multi-level dual attention-based network for self-supervised monocular depth estimation. IEEE Transactions on Image Processing, 30, 4691-4705.

\bibitem{scene_Multimodal_scale_consistency}
Chawla, H., Varma, A., Arani, E., & Zonooz, B. (2021, May). Multimodal scale consistency and awareness for monocular self-supervised depth estimation. In 2021 IEEE International Conference on Robotics and Automation (ICRA) (pp. 5140-5146). IEEE.

\bibitem{scene_Channel_Wise_Attention_Based_Network}
Yan, J., Zhao, H., Bu, P., & Jin, Y. (2021, December). Channel-Wise Attention-Based Network for Self-Supervised Monocular Depth Estimation. In 2021 International Conference on 3D Vision (3DV) (pp. 464-473). IEEE.

\bibitem{scene_Transformers_in_Self_Supervised_Monocular_Depth_Estimation}
Varma, A., Chawla, H., Zonooz, B., & Arani, E. (2022). Transformers in Self-Supervised Monocular Depth Estimation with Unknown Camera Intrinsics. arXiv preprint arXiv:2202.03131.

\bibitem{scene_SideRT}
Shu, C., Chen, Z., Chen, L., Ma, K., Wang, M., & Ren, H. (2022). SideRT: A Real-time Pure Transformer Architecture for Single Image Depth Estimation. arXiv preprint arXiv:2204.13892.

\bibitem{scene_DepthFormer}
Li, Z., Chen, Z., Liu, X., & Jiang, J. (2022). DepthFormer: Exploiting Long-Range Correlation and Local Information for Accurate Monocular Depth Estimation. arXiv preprint arXiv:2203.14211.



%%%%HDmap%%%
\bibitem{HDmap_79}
M. Javanmardi et al., “Towards high-definition 3D urban mapping: Road feature-based registration of mobile mapping systems and aerial imagery,” Remote Sens., vol. 9, no. 10, p. 975, 2017.

\bibitem{HDmap_80}
K. Wong, E. Javanmardi, M. Javanmardi, and S. Kamijo, “Estimating autonomous vehicle localization error using 2D geographic information,” ISPRS Int. J. Geo-Inform., vol. 8, no. 6, p. 288, 2019.

\bibitem{HDmap_34}
M. Javanmardi et al., “Towards high-definition 3D urban mapping:Road feature-based registration of mobile mapping systems and aer-
ial imagery,” Remote Sens., vol. 9, no. 10, p. 975, 2017. 

\bibitem{HDmap_54}
M. Javanmardi et al., “Towards high-definition 3D urban mapping:Road feature-based registration of mobile mapping systems and aer-
ial imagery,” Remote Sens., vol. 9, no. 10, p. 975, 2017.
%%%planning%%%
\bibitem{planning_1}
Katrakazas, M. Quddus, W. Chen, and L. Deka, “Real-time motion planning methods for autonomous on-road driving: State-of-the-art and future research directions,” {\it{Transportation Research Part C: Emerging Technologies}}, vol. 60, pp. 416 - 442, 2015.
\bibitem{planning_2}
Paden, B., Čáp, M., Yong, S. Z., Yershov, D., & Frazzoli, E. (2016). A survey of motion planning and control techniques for self-driving urban vehicles. {\it{IEEE Transactions on intelligent vehicles}}, 1(1), 33-55.
\bibitem{planning_3}
L. Claussmann, M. Revilloud, D. Gruyer, et al., “A review of motion planning for highway autonomous driving,” {\it{IEEE Transactions on Intelligent Transportation Systems}}, vol. 21, no. 5, pp. 1826–1848, 2020.
\bibitem{planning_4}
H. Bast, D. Delling, A. Goldberg, et al., Route planning in transportation networks, in Algorithm Engineering. Cham, Switzerland: Springer, 2016, pp. 19–80.
\bibitem{planning_5}
D. Delling, P. Sanders, D. Schultes, and D. Wagner, “Engineering route planning algorithms,” in Algorithmics of Large and Complex Networks. Springer, 2009, pp. 117–139.
\bibitem{planning_6}
B. Li, Z. Yin, Y. Ouyang, et al.,  "Online trajectory replanning for sudden environmental changes during automated parking: A parallel stitching method," {\it{IEEE Transactions on Intelligent Vehicles}}, 2022.
\bibitem{planning_7}
Y. Huang, H. Ding, Y. Zhang, et al., A motion planning and tracking framework for autonomous vehicles based on artificial potential field elaborated resistance network approach. {\it{IEEE Transactions on Industrial Electronics}}, 67(2), 1376-1386, 2019.
\bibitem{planning_8}
Hoel, C. J., Driggs-Campbell, K., Wolff, K., Laine, L., & Kochenderfer, M. J. (2019). Combining planning and deep reinforcement learning in tactical decision making for autonomous driving. {\it{IEEE transactions on intelligent vehicles}}, 5(2), 294-305.
\bibitem{planning_9}
M. Montemerlo, J. Becker, S. Bhat, et al., (2008). Junior: The stanford entry in the urban challenge. {\it{Journal of Field Robotics}}, 25(9), 569-597.
\bibitem{planning_10}
Y. Liu, X. Hu, G. Chen, et al., Review of end-to-end motion planning for autonomous driving with visual perception.{\it{ Journal of Image and Graphics}}, 26(01): 49-66. 2021.
\bibitem{planning_11}
Rehder, E., Quehl, J., & Stiller, C. (2017, September). Driving like a human: Imitation learning for path planning using convolutional neural networks. {\it{In International Conference on Robotics and Automation Workshops}} (pp. 1-5).
\bibitem{planning_12}
Chen, L., Hu, X., Tian, W., Wang, H., Cao, D., & Wang, F. Y. (2018). Parallel planning: A new motion planning framework for autonomous driving. {\it{IEEE/CAA Journal of Automatica Sinica}}, 6(1), 236-246.
\bibitem{planning_13}
Zhang, X., Jiang, Y., Lu, Y., & Xu, X. (2022). A Receding-Horizon Reinforcement Learning Approach for Kinodynamic Motion Planning of Autonomous Vehicles. {\it{IEEE Transactions on Intelligent Vehicles}}.
\bibitem{planning_14}
Kendall, A., Hawke, J., Janz, D., Mazur, P., Reda, D., Allen, J. M., ... & Shah, A. (2019, May). Learning to drive in a day. {\it{In 2019 International Conference on Robotics and Automation (ICRA)}} (pp. 8248-8254). IEEE.
\bibitem{planning_15}
Aradi, S. (2020). Survey of deep reinforcement learning for motion planning of autonomous vehicles. {\it{IEEE Transactions on Intelligent Transportation Systems}}. vol. 23, no. 2, pp. 740 - 759.
\bibitem{planning_16}
B. Li, T. Acarman, Y. Zhang, et al., “Optimization-based trajectory planning for autonomous parking with irregularly placed obstacles: A lightweight iterative framework,” {\it{IEEE Transactions on Intelligent Transportation Systems}}, 2021.
\bibitem{planning_17}
D. Dolgov, S. Thrun, M. Montemerlo, and J. Diebel, “Path planning for autonomous vehicles in unknown semi-structured environments,” Int. {\it{Journal of Robotics Research}}, vol. 29, no. 5, pp. 485–501, 2010.
\bibitem{planning_18}
Fassbender, D., Heinrich, B. C., & Wuensche, H. J. (2016, October). Motion planning for autonomous vehicles in highly constrained urban environments. In 2016 {\it{IEEE/RSJ international conference on intelligent robots and systems (IROS)}} (pp. 4708-4713). IEEE.
\bibitem{planning_19}
W. Xu, J. Pan, J. Wei, and J. M. Dolan, “Motion planning under uncertainty for on-road autonomous driving,” In Proc. 2014 {\it{IEEE International Conference on Robotics and Automation (ICRA)}}, pp. 2507–2512, 2014.
\bibitem{planning_20}
M. McNaughton, C. Urmson, J. M. Dolan, and J. Lee, “Motion planning for autonomous driving with a conformal spatiotemporal lattice,” In Proc. 2011 {\it{IEEE International Conference on Robotics and Automation (ICRA)}}, pp. 4889–4895, 2011.
\bibitem{planning_21}
H. Fan, F. Zhu, C. Liu, et al., “Baidu Apollo EM motion planner,” arXiv preprint, available at https://arxiv.org/abs/1807.08048, 2018.
\bibitem{planning_22}
X. Li, Z. Sun, D. Cao, et al., “Real-time trajectory planning for autonomous urban driving: framework, algorithms, and verifications,” {\it{IEEE/ASME Transactions on Mechatronics}}, vol. 21, no. 2, pp. 740–753, 2016.
\bibitem{planning_23}H. Bai, S. Cai, N. Ye, et al., (2015, May). Intention-aware online POMDP planning for autonomous driving in a crowd. In 2015 {\it{ieee international conference on robotics and automation (icra)}} (pp. 454-460). IEEE.
\bibitem{planning_24}
Ye, N., Somani, A., Hsu, D., & Lee, W. S. (2017). DESPOT: Online POMDP planning with regularization. {\it{Journal of Artificial Intelligence Research}}, 58, 231-266.
\bibitem{planning_25}
K. Kondak, and G. Hommel, “Computation of time-optimal movements for autonomous parking of non-holonomic mobile platforms,” In Proc. 2001 {\it{IEEE International Conference on Robotics and Automation}}, vol. 3, pp. 2698–2703, 2001.
\bibitem{planning_26}
X. Zhang, A. Liniger, A. Sakai, and F. Borrelli, “Autonomous parking using optimization-based collision avoidance,” In Proc. 2018 {\it{IEEE Conference on Decision and Control}}, pp. 4327–4332, 2018.
\bibitem{planning_27}
J. Chen, W. Zhan, and M. Tomizuka, “Autonomous driving motion planning with constrained iterative LQR,” {\it{IEEE Transactions on Intelligent Vehicles}}, vol. 4, no. 2, pp. 244–254, 2019.
\bibitem{planning_28}
A. Liniger, A. Domahidi, and M. Morari, “Optimization-based autonomous racing of 1:43 scale RC cars”, {\it{Optimal Control Applications and Methods}}, pp. 628–647, 2015.
\bibitem{planning_29}
B. Li, Y. Ouyang, L. Li and Y. Zhang, "Autonomous driving on curvy roads without reliance on Frenet frame: A cartesian-based trajectory planning method," {\it{IEEE Transactions on Intelligent Transportation Systems}}, doi: 10.1109/TITS.2022.3145389.
\bibitem{planning_30}
W. Lim, S. Lee, M. Sunwoo, et al., “Hierarchical trajectory planning of an autonomous car based on the integration of a sampling and an optimization method,” {\it{IEEE Transactions on Intelligent Transportation Systems}}, vol. 19, no. 2, pp. 613–626, 2018.
\bibitem{planning_31}
Scheffe, P., Henneken, T. M., Kloock, M., & Alrifaee, B. (2022). Sequential convex programming methods for real-time optimal trajectory planning in autonomous vehicle racing. {\it{IEEE Transactions on Intelligent Vehicles}}.
\bibitem{planning_32}
Miller, C., Pek, C., & Althoff, M. (2018, June). Efficient mixed-integer programming for longitudinal and lateral motion planning of autonomous vehicles. In 2018 {\it{IEEE Intelligent Vehicles Symposium (IV)}} (pp. 1954-1961). IEEE.
\bibitem{planning_33}
Claussmann, L., Revilloud, M., & Glaser, S. (2019, May). Simulated annealing-optimized trajectory planning within non-collision nominal intervals for highway autonomous driving. In 2019 {\it{International Conference on Robotics and Automation (ICRA)}} (pp. 5922-5928). IEEE.
\bibitem{planning_34}
Quinlan, S., & Khatib, O. (1993, May). Elastic bands: Connecting path planning and control. In [1993] {\it{Proceedings IEEE International Conference on Robotics and Automation}} (pp. 802-807). IEEE.
\bibitem{planning_35}
Rösmann, C., Hoffmann, F., & Bertram, T. (2017). Integrated online trajectory planning and optimization in distinctive topologies. {\it{Robotics and Autonomous Systems}}, 88, 142-153.
\bibitem{planning_36}
Hang, P., Lv, C., Huang, C., Cai, J., Hu, Z., & Xing, Y. (2020). An integrated framework of decision making and motion planning for autonomous vehicles considering social behaviors. {\it{IEEE transactions on vehicular technology}}, 69(12), 14458-14469.
\bibitem{planning_37}
Gu, T., Atwood, J., Dong, C., Dolan, J. M., & Lee, J. W. (2015, September). Tunable and stable real-time trajectory planning for urban autonomous driving. In 2015 {\it{IEEE/RSJ international conference on intelligent robots and systems (IROS)}} (pp. 250-256). IEEE.
\bibitem{planning_38}
D. Le, Z. Liu, J. Jin, K. Zhang, and B. Zhang, “Historical improvement optimal motion planning with model predictive trajectory optimization for on-road autonomous vehicle,” In Proc. 45th {\it{Annual Conference of IEEE Industrial Electronics Society}}, pp. 5223–5230, 2019.
\bibitem{planning_39}
Park, J., Karumanchi, S., & Iagnemma, K. (2015). Homotopy-based divide-and-conquer strategy for optimal trajectory planning via mixed-integer programming. {\it{IEEE Transactions on Robotics}}, 31(5), 1101-1115.
\bibitem{planning_40}
J. Ziegler, P. Bender, T. Dang, et al., “Trajectory planning for Bertha — A local, continuous method,” In Proc. 2014 {\it{IEEE Intelligent Vehicles Symposium (IV)}}, pp. 450–457, 2014.
\bibitem{planning_41}
Dubins, L. E. (1957). On curves of minimal length with a constraint on average curvature, and with prescribed initial and terminal positions and tangents. {\it{American Journal of mathematics}}, 79(3), 497-516.
\bibitem{planning_42}
Reeds, J., & Shepp, L. (1990). Optimal paths for a car that goes both forwards and backwards. {\it{Pacific journal of mathematics}}, 145(2), 367-393.
\bibitem{planning_43}
M. Werling, J. Ziegler, S. Kammel, et al., “Optimal trajectory generation for dynamic street scenarios in a Frenet frame,” In Proc. 2010 {\it{IEEE International Conference on Robotics and Automation (ICRA)}}, pp. 987–993, 2010.
\bibitem{planning_44}
Patten, W. N., Wu, H. C., & Cai, W. (1994). Perfect parallel parking via Pontryagin's principle. J. Dyn. Sys., Meas., Control. Dec 1994, 116(4): 723-728.
\bibitem{planning_45}
Y. Kuwata, J. Teo, G. Fiore, et al., “Real-time motion planning with applications to autonomous urban driving,” {\it{IEEE Transactions on Control Systems Technology}}, vol. 17, no. 5, pp. 1105–1118, 2009.
\bibitem{planning_46}
Y. Zhang, H. Chen, S. Waslander, et al., “Hybrid trajectory planning for autonomous driving in highly constrained environments,” {\it{IEEE Access}}, vol. 6, pp. 32800–32819, 2018.
\bibitem{planning_47}
M. Rufli, and R. Siegwart, “On the design of deformable input-/ state-lattice graphs,” In Proc. 2010 {\it{IEEE International Conference on Robotics and Automation}}, pp. 3071–3077, 2010.
\bibitem{planning_48}
Bergman, K., Ljungqvist, O., & Axehill, D. (2020). Improved path planning by tightly combining lattice-based path planning and optimal control. {\it{IEEE Transactions on Intelligent Vehicles}}, 6(1), 57-66.
\bibitem{planning_49}
Liu, C., Zhan, W., & Tomizuka, M. (2017, June). Speed profile planning in dynamic environments via temporal optimization. In 2017 {\it{IEEE Intelligent Vehicles Symposium (IV)}} (pp. 154-159). IEEE.
\bibitem{planning_50}
L. Ma, J. Xue, K. Kawabata, et al., “Efficient sampling-based motion planning for on-road autonomous driving,” {\it{IEEE Transactions on Intelligent Transportation Systems}}, vol. 16, no. 4, pp. 1961–1976, 2015.
\bibitem{planning_51}
Tian, F., Zhou, R., Li, Z., Li, L., Gao, Y., Cao, D., & Chen, L. (2022). Trajectory planning for autonomous mining trucks considering terrain constraints. {\it{IEEE Transactions on Intelligent Vehicles}}, 6(4), 772-786.
\bibitem{planning_52}
Müller, J., & Buchholz, M. (2019, October). A risk and comfort optimizing motion planning scheme for merging scenarios. In 2019 {\it{IEEE Intelligent Transportation Systems Conference (ITSC)}} (pp. 3155-3161). IEEE.
\bibitem{planning_53}
Hubmann, C., Schulz, J., Becker, M., Althoff, D., & Stiller, C. (2018). Automated driving in uncertain environments: Planning with interaction and uncertain maneuver prediction. {\it{IEEE transactions on intelligent vehicles}}, 3(1), 5-17.
\bibitem{planning_54}
Andersen, H., Alonso-Mora, J., Eng, Y. H., Rus, D., & Ang, M. H. (2019). Trajectory optimization and situational analysis framework for autonomous overtaking with visibility maximization. {\it{IEEE Transactions on Intelligent Vehicles}}, 5(1), 7-20.
\bibitem{planning_55}
Pek, C., & Althoff, M. (2020). Fail-safe motion planning for online verification of autonomous vehicles using convex optimization. {\it{IEEE Transactions on Robotics}}, 37(3), 798-814.


%%%%%%system%%%%%%%%%%%
\bibitem{system_1}
Liu, Liangkai, et al. "Computing systems for autonomous driving: State of the art and challenges." IEEE Internet of Things Journal 8.8 (2020): 6469-6486.
\bibitem{system_2}
Muller, Urs, et al. "Off-road obstacle avoidance through end-to-end learning." Advances in neural information processing systems 18 (2005). 
\bibitem{system_3}
Kendall, Alex, et al. "Learning to drive in a day." 2019 International Conference on Robotics and Automation (ICRA). IEEE, 2019.
\bibitem{system_4}
Liu, Shaoshan, et al. "Edge computing for autonomous driving: Opportunities and challenges." Proceedings of the IEEE 107.8 (2019): 1697-1716.
\bibitem{system_5}
Lin, Shih-Chieh, et al. "The architectural implications of autonomous driving: Constraints and acceleration." Proceedings of the Twenty-Third International Conference on Architectural Support for Programming Languages and Operating Systems. 2018.
\bibitem{system_6}
Liu, Shaoshan, et al. "Computer architectures for autonomous driving." Computer 50.8 (2017): 18-25.
\bibitem{system_7}
Wu, Tianze, et al. "Oops! It's Too Late. Your Autonomous Driving System Needs a Faster Middleware." IEEE Robotics and Automation Letters 6.4 (2021): 7301-7308.
\bibitem{system_8}
Yeong, De Jong, et al. "Sensor and sensor fusion technology in autonomous vehicles: A review." Sensors 21.6 (2021): 2140.
\bibitem{system_9}
Jagannadha, Pavan Kumar Datla, et al. "Special session: in-system-test (IST) architecture for Nvidia drive-AGX platforms." 2019 IEEE 37th VLSI Test Symposium (VTS). IEEE, 2019. 
\bibitem{system_10}
Boppana, Vamsi, et al. "UltraScale+ MPSoC and FPGA families." 2015 IEEE Hot Chips 27 Symposium (HCS). IEEE, 2015. 
\bibitem{system_11}
Jouppi, Norman P., et al. "Ten lessons from three generations shaped google’s tpuv4i: Industrial product." 2021 ACM/IEEE 48th Annual International Symposium on Computer Architecture (ISCA). IEEE, 2021.
\bibitem{system_12}
Hildebrand, Dan. "An Architectural Overview of QNX." USENIX Workshop on Microkernels and Other Kernel Architectures. 1992.
\bibitem{system_13}
Hambarde, Prasanna, Rachit Varma, and Shivani Jha. "The survey of real time operating system: RTOS." 2014 International Conference on Electronic Systems, Signal Processing and Computing Technologies. IEEE, 2014. Wu, Tianze, et al. 
\bibitem{system_14}
Wu, Tianze, et al. "Oops! It's Too Late. Your Autonomous Driving System Needs a Faster Middleware." IEEE Robotics and Automation Letters 6.4 (2021): 7301-7308. 
\bibitem{system_15}
Quigley, Morgan, et al. "ROS: an open-source Robot Operating System." ICRA workshop on open source software. Vol. 3. No. 3.2. 2009.
\bibitem{system_16}
DiLuoffo, Vincenzo, William R. Michalson, and Berk Sunar. "Robot Operating System 2: The need for a holistic security approach to robotic architectures." International Journal of Advanced Robotic Systems 15.3 (2018): 1729881418770011.
\bibitem{system_17}
Fayazbakhsh, Mohammad Ali, and Majid Bahrami. "Comprehensive modeling of vehicle air conditioning loads using heat balance method." SAE technical paper 2013 (2013): 1507.
\bibitem{system_18}
Farrington, Rob, and John Rugh. Impact of vehicle air-conditioning on fuel economy, tailpipe emissions, and electric vehicle range. No. NREL/CP-540-28960. National Renewable Energy Lab.(NREL), Golden, CO (United States), 2000.
\bibitem{system_19}
Fayyad, Jamil, et al. "Deep learning sensor fusion for autonomous vehicle perception and localization: A review." Sensors 20.15 (2020): 4220.
\bibitem{system_20}
Wang, Zhangjing, Yu Wu, and Qingqing Niu. "Multi-sensor fusion in automated driving: A survey." Ieee Access 8 (2019): 2847-2868.
\bibitem{system_21}
Marti, Enrique, et al. "A review of sensor technologies for perception in automated driving." IEEE Intelligent Transportation Systems Magazine 11.4 (2019): 94-108.
\bibitem{system_22}
Badue, Claudine, et al. "Self-driving cars: A survey." Expert Systems with Applications 165 (2021): 113816.
\bibitem{system_23}
Li, Ying, et al. "Deep learning for lidar point clouds in autonomous driving: A review." IEEE Transactions on Neural Networks and Learning Systems 32.8 (2020): 3412-3432.
\bibitem{system_24}
Wang, Dingkang, Connor Watkins, and Huikai Xie. "MEMS mirrors for LiDAR: a review." Micromachines 11.5 (2020): 456.
\bibitem{system_25}
Hsu, Ching-Pai, et al. "A review and perspective on optical phased array for automotive LiDAR." IEEE Journal of Selected Topics in Quantum Electronics 27.1 (2020): 1-16.
\bibitem{system_26}
Elhousni, Mahdi, and Xinming Huang. "A survey on 3d lidar localization for autonomous vehicles." 2020 IEEE Intelligent Vehicles Symposium (IV). IEEE, 2020.
\bibitem{system_27}
Royo, Santiago, and Maria Ballesta-Garcia. "An overview of lidar imaging systems for autonomous vehicles." Applied Sciences 9.19 (2019): 4093.
\bibitem{system_28}
Van Nam, Dinh, and Kim Gon-Woo. "Solid-state LiDAR based-SLAM: A concise review and application." 2021 IEEE International Conference on Big Data and Smart Computing (BigComp). IEEE, 2021.
\bibitem{system_29}
Cui, Yaodong, et al. "Deep learning for image and point cloud fusion in autonomous driving: A review." IEEE Transactions on Intelligent Transportation Systems (2021).
\bibitem{system_30}
Van Brummelen, Jessica, et al. "Autonomous vehicle perception: The technology of today and tomorrow." Transportation research part C: emerging technologies 89 (2018): 384-406.
\bibitem{system_31}
Fayyad, Jamil, et al. "Deep learning sensor fusion for autonomous vehicle perception and localization: A review." Sensors 20.15 (2020): 4220.
\bibitem{system_32}
Debeunne, César, and Damien Vivet. "A review of visual-LiDAR fusion based simultaneous localization and mapping." Sensors 20.7 (2020): 2068.
\bibitem{system_33}
Zhou, Taohua, et al. "MMW radar-based technologies in autonomous driving: A review." Sensors 20.24 (2020): 7283.
\bibitem{system_34}
Wei, Zhiqing, et al. "MmWave Radar and Vision Fusion for Object Detection in Autonomous Driving: A Review." Sensors 22.7 (2022): 2542.
\bibitem{system_35}
Ma, Dingyou, et al. "Joint radar-communication strategies for autonomous vehicles: Combining two key automotive technologies." IEEE signal processing magazine 37.4 (2020): 85-97.
\bibitem{system_36}
Saponara, Sergio, Maria Sabrina Greco, and Fulvio Gini. "Radar-on-chip/in-package in autonomous driving vehicles and intelligent transport systems: Opportunities and challenges." IEEE Signal Processing Magazine 36.5 (2019): 71-84.
\bibitem{system_37}
Javadi, S. Hamed, and Alfonso Farina. "Radar networks: A review of features and challenges." Information fusion 61 (2020): 48-55.
\bibitem{system_38}
Mousazadeh, Hossein. "A technical review on navigation systems of agricultural autonomous off-road vehicles." Journal of Terramechanics 50.3 (2013): 211-232.
\bibitem{system_39}
Jing, Hao, et al. "Integrity Monitoring of GNSS/INS Based Positioning Systems for Autonomous Vehicles: State-of-the-Art and Open Challenges." IEEE Transactions on Intelligent Transportation Systems (2022). 
\bibitem{system_40}
Rosique, Francisca, et al. "A systematic review of perception system and simulators for autonomous vehicles research." Sensors 19.3 (2019): 648.
\bibitem{system_41}
Mohammed, Abdul Sajeed, et al. "The perception system of intelligent ground vehicles in all weather conditions: a systematic literature review." Sensors 20.22 (2020): 6532.
\bibitem{system_42}
Xing, Yang, et al. "Advances in vision-based lane detection: algorithms, integration, assessment, and perspectives on ACP-based parallel vision." IEEE/CAA Journal of Automatica Sinica 5.3 (2018): 645-661.
\bibitem{system_43}
Zhang, Hao, et al. "Image fusion meets deep learning: A survey and perspective." Information Fusion 76 (2021): 323-336.
\bibitem{system_44}
Kedem, Benjamin, Victor De Oliveira, and Michael Sverchkov. "Statistical data fusion." (2017).
\bibitem{system_45}
Berrio, Julie Stephany, et al. "Camera-LIDAR integration: Probabilistic sensor fusion for semantic mapping." IEEE Transactions on Intelligent Transportation Systems (2021).
\bibitem{system_46}
Sasiadek, J. Z., and P. Hartana. "Sensor data fusion using Kalman filter." Proceedings of the Third International Conference on Information Fusion. Vol. 2. IEEE, 2000.
\bibitem{system_47}
https://www.bsigroup.com/globalassets/localfiles/en-gb/cav/cav-standards-roadmap/cav-standards-roadmap-2022.pdf.
\bibitem{system_48}
Gao, Yu, Yunfeng Ai, Bin Tian, Long Chen, Jian Wang, Dongpu Cao, and Fei-Yue Wang. "Parallel end-to-end autonomous mining: An IoT-oriented approach." IEEE Internet of Things Journal 7, no. 2 (2019): 1011-1023.
\bibitem{system_49}
Hájnik, Ambróz, Veronika Harantová, and Alica Kalašová. "Use of electromobility and autonomous vehicles at airports in Europe and worldwide." Transportation Research Procedia 55 (2021): 71-78.
\bibitem{system_50}
Uhlemann, Elisabeth. "Autonomous Vehicles Have Entered the Off-Road Market [Connected and Automated Vehicles]." IEEE Vehicular Technology Magazine 16.2 (2021): 15-19.
\bibitem{system_51}
Van Meldert, Bram, and Liesje De Boeck. "Introducing autonomous vehicles in logistics: a review from a broad perspective." FEB Research Report KBI_1618 (2016).
\bibitem{system_52}
Omeiza, Daniel, et al. "Explanations in autonomous driving: A survey." IEEE Transactions on Intelligent Transportation Systems (2021).
\bibitem{system_53}
Zablocki, Éloi, et al. "Explainability of vision-based autonomous driving systems: Review and challenges." arXiv preprint arXiv:2101.05307 (2021).
\bibitem{system_54}Atakishiyev, Shahin, et al. "Explainable Artificial Intelligence for Autonomous Driving: A Comprehensive Overview and Field Guide for Future Research Directions." arXiv preprint arXiv:2112.11561 (2021).

@article{paden2016survey,
  title={A survey of motion planning and control techniques for self-driving urban vehicles},
  author={Paden, Brian and {\v{C}}{\'a}p, Michal and Yong, Sze Zheng and Yershov, Dmitry and Frazzoli, Emilio},
  journal={IEEE Transactions on intelligent vehicles},
  volume={1},
  number={1},
  pages={33--55},
  year={2016},
  publisher={IEEE}
}

@inproceedings{prediction1,
  title={Desire: Distant future prediction in dynamic scenes with interacting agents},
  author={Lee, Namhoon and Choi, Wongun and Vernaza, Paul and Choy, Christopher B and Torr, Philip HS and Chandraker, Manmohan},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={336--345},
  year={2017}
}
@inproceedings{prediction2,
  title={Probabilistic prediction of vehicle semantic intention and motion},
  author={Hu, Yeping and Zhan, Wei and Tomizuka, Masayoshi},
  booktitle={2018 IEEE Intelligent Vehicles Symposium (IV)},
  pages={307--313},
  year={2018},
  organization={IEEE}
}
@inproceedings{prediction3,
  title={Fast and furious: Real time end-to-end 3d detection, tracking and motion forecasting with a single convolutional net},
  author={Luo, Wenjie and Yang, Bin and Urtasun, Raquel},
  booktitle={Proceedings of the IEEE conference on Computer Vision and Pattern Recognition},
  pages={3569--3577},
  year={2018}
}

@ARTICLE{Kalman1,
  author={Guo, Ge and Zhao, Shijie},
  journal={IEEE Transactions on Intelligent Vehicles}, 
  title={3D Multi-Object Tracking with Adaptive Cubature Kalman Filter for Autonomous Driving}, 
  year={2022},
  volume={},
  number={},
  pages={1-1},
  doi={10.1109/TIV.2022.3158419}}
  
@ARTICLE{Kalman2,
  author={Bahramgiri, Mojtaba and Nooshabadi, Saeid and Olutomilayo, Kunle and Fuhrmann, Daniel},
  journal={IEEE Transactions on Intelligent Vehicles}, 
  title={Automotive Radar-Based Hitch Angle Tracking Technique for Trailer Backup Assistant Systems}, 
  year={2022},
  volume={},
  number={},
  pages={1-1},
  doi={10.1109/TIV.2022.3144896}}
  
@ARTICLE{Kalman3,
  author={Xie, Zhenming and Jeon, Woongsun and Rajamani, Rajesh},
  journal={IEEE Transactions on Intelligent Vehicles}, 
  title={Low-Density Lidar Based Estimation System for Bicycle Protection}, 
  year={2021},
  volume={6},
  number={1},
  pages={67-77},
  doi={10.1109/TIV.2020.3010728}}
  
@ARTICLE{graph1,
  author={Lv, Hui and Liu, Chao and Zhao, Xiaowei and Xu, Chunyan and Cui, Zhen and Yang, Jian},
  journal={IEEE Transactions on Intelligent Vehicles}, 
  title={Lane Marking Regression From Confidence Area Detection to Field Inference}, 
  year={2021},
  volume={6},
  number={1},
  pages={47-56},
  doi={10.1109/TIV.2020.3009366}}
  


@ARTICLE{graph3,
  author={Zhao, Chengfeng and Fu, Chen and Dolan, John M. and Wang, Jun},
  journal={IEEE Transactions on Intelligent Vehicles}, 
  title={L-Shape Fitting-Based Vehicle Pose Estimation and Tracking Using 3D-LiDAR}, 
  year={2021},
  volume={6},
  number={4},
  pages={787-798},
  doi={10.1109/TIV.2021.3078619}}
  
@ARTICLE{TrackingNetwork1,
  author={Zhu, Yabin and Li, Chenglong and Tang, Jin and Luo, Bin},
  journal={IEEE Transactions on Intelligent Vehicles}, 
  title={Quality-Aware Feature Aggregation Network for Robust RGBT Tracking}, 
  year={2021},
  volume={6},
  number={1},
  pages={121-130},
  doi={10.1109/TIV.2020.2980735}}
  
@ARTICLE{TrackingNetwork2,
  author={Hoffmann, João Eduardo and Tosso, Hilkija Gaïus and Santos, Max Mauro Dias and Justo, João Francisco and Malik, Asad Waqar and Rahman, Anis Ur},
  journal={IEEE Transactions on Intelligent Vehicles}, 
  title={Real-Time Adaptive Object Detection and Tracking for Autonomous Vehicles}, 
  year={2021},
  volume={6},
  number={3},
  pages={450-459},
  doi={10.1109/TIV.2020.3037928}}
  
@inproceedings{TrackingLSTM1,
  title={Online multi-target tracking using recurrent neural networks},
  author={Milan, Anton and Rezatofighi, S Hamid and Dick, Anthony and Reid, Ian and Schindler, Konrad},
  booktitle={Thirty-First AAAI conference on artificial intelligence},
  year={2017}
}

@inproceedings{TrackingLSTM2,
  title={Probabilistic vehicle trajectory prediction over occupancy grid map via recurrent neural network},
  author={Kim, ByeoungDo and Kang, Chang Mook and Kim, Jaekyum and Lee, Seung Hi and Chung, Chung Choo and Choi, Jun Won},
  booktitle={2017 IEEE 20th International Conference on Intelligent Transportation Systems (ITSC)},
  pages={399--404},
  year={2017},
  organization={IEEE}
}



% human-machine
\bibitem{human-machine_1}Hasenjäger, Martina, Martin Heckmann, and Heiko Wersing. "A survey of personalization for advanced driver assistance systems." IEEE Transactions on Intelligent Vehicles 5.2 (2019): 335-344.
\bibitem{human-machine_2}Xing, Yang, Chen Lv, Dongpu Cao, and Peng Hang. "Toward human-vehicle collaboration: Review and perspectives on human-centered collaborative automated driving." Transportation research part C: emerging technologies 128 (2021): 103199.
\bibitem{human-machine_3}Wang, Wenshuo, and Ding Zhao. "Evaluation of lane departure correction systems using a regenerative stochastic driver model." IEEE Transactions on Intelligent Vehicles 2.3 (2017): 221-232.
\bibitem{human-machine_4}Chen, Wuwei, et al. "Human–machine shared control for lane departure assistance based on hybrid system theory." Control Engineering Practice 84 (2019): 399-407.
\bibitem{human-machine_5}Althoff, Matthias, Sebastian Maierhofer, and Christian Pek. "Provably-correct and comfortable adaptive cruise control." IEEE Transactions on Intelligent Vehicles 6.1 (2020): 159-174.
\bibitem{human-machine_6}Utriainen, Roni, Markus Pöllänen, and Heikki Liimatainen. "The safety potential of lane keeping assistance and possible actions to improve the potential." IEEE Transactions on Intelligent Vehicles 5.4 (2020): 556-564.
\bibitem{human-machine_7}Lal, Saroj KL, and Ashley Craig. "A critical review of the psychophysiology of driver fatigue." Biological psychology 55.3 (2001): 173-194.
\bibitem{human-machine_8}Xing, Yang, et al. "Driver lane change intention inference for intelligent vehicles: framework, survey, and challenges." IEEE Transactions on Vehicular Technology 68.5 (2019): 4377-4390.
\bibitem{human-machine_9}Hu, Zhongxu, et al. "Data-driven estimation of driver attention using calibration-free eye gaze and scene features." IEEE Transactions on Industrial Electronics 69.2 (2021): 1800-1808.
\bibitem{human-machine_10}Marquart, Gerhard, Christopher Cabrall, and Joost de Winter. "Review of eye-related measures of drivers’ mental workload." Procedia Manufacturing 3 (2015): 2854-2861.
\bibitem{human-machine_11}Zepf, Sebastian, et al. "Driver emotion recognition for intelligent vehicles: A survey." ACM Computing Surveys (CSUR) 53.3 (2020): 1-30.
\bibitem{human-machine_12}Kashevnik, Alexey, et al. "Driver distraction detection methods: A literature review and framework." IEEE Access 9 (2021): 60063-60076.
\bibitem{human-machine_13}Balandong, Rodney Petrus, et al. "A review on EEG-based automatic sleepiness detection systems for driver." Ieee Access 6 (2018): 22908-22919.
\bibitem{human-machine_14}Xing, Yang, Chen Lv, Yifan Zhao, Yahui Liu, Dongpu Cao, and Sadahiro Kawahara. "Pattern recognition and characterization of upper limb neuromuscular dynamics during driver-vehicle interactions." Iscience 23, no. 9 (2020): 101541.
\bibitem{human-machine_15}Zhongxu Hu, et al. Review and Perspectives on Driver Digital Twin and Its Enabling Technologies for Intelligent Vehicles. IEEE Trans. on Intelligent Vehicles. 2022.
\bibitem{human-machine_16}Du, Na, et al. "Predicting driver takeover performance in conditionally automated driving." Accident Analysis & Prevention 148 (2020): 105748.
\bibitem{human-machine_17}Weaver, Bradley W., and Patricia R. DeLucia. "A systematic review and meta-analysis of takeover performance during conditionally automated driving." Human factors (2020): 0018720820976476.
\bibitem{human-machine_18}Louw, Tyron, et al. "Driver inattention during vehicle automation: How does driver engagement affect resumption of control?." 4th International Conference on Driver Distraction and Inattention (DDI2015), Sydney: proceedings. ARRB Group, 2015.
\bibitem{human-machine_19}Salubre, Kevin Joel, and Dan Nathan-Roberts. "Takeover request design in automated driving: a systematic review." Proceedings of the Human Factors and Ergonomics Society Annual Meeting. Vol. 65. No. 1. Sage CA: Los Angeles, CA: SAGE Publications, 2021.
\bibitem{human-machine_20}Eriksson, Alexander, and Neville A. Stanton. "Takeover time in highly automated vehicles: noncritical transitions to and from manual control." Human factors 59.4 (2017): 689-705.
\bibitem{human-machine_21}Hu, Zhongxu, et al. "Driver Anomaly Quantification for Intelligent Vehicles: A Contrastive Learning Approach with Representation Clustering." IEEE Transactions on Intelligent Vehicles (2022).
\bibitem{human-machine_22}Lv, Chen, et al. "Human–Machine Collaboration for Automated Driving Using an Intelligent Two‐Phase Haptic Interface." Advanced Intelligent Systems 3.4 (2021): 2000229.
\bibitem{human-machine_23}Jing, Peng, et al. "The Determinants behind the Acceptance of Autonomous Vehicles: A Systematic Review." Sustainability 12.5 (2020): 1719.
\bibitem{human-machine_24}Olaverri-Monreal, Cristina. "Promoting trust in self-driving vehicles." Nature Electronics 3.6 (2020): 292-294.
\bibitem{human-machine_25}Choi, Jong Kyu, and Yong Gu Ji. "Investigating the importance of trust in adopting an autonomous vehicle." International Journal of Human-Computer Interaction 31.10 (2015): 692-702.
\bibitem{human-machine_26}Dikmen, Murat, and Catherine Burns. "Trust in autonomous vehicles: The case of tesla autopilot and summon." 2017 IEEE International Conference on Systems, Man, and Cybernetics (SMC). IEEE, 2017.
\bibitem{human-machine_27}Ayoub, Jackie, et al. "From manual driving to automated driving: A review of 10 years of autoui." Proceedings of the 11th International Conference on Automotive User Interfaces and Interactive Vehicular Applications. 2019.
\bibitem{human-machine_28}Liu, Weimin, et al. "A Literature Review on Additional Semantic Information Conveyed from Driving Automation Systems to Drivers through Advanced In-Vehicle HMI Just Before, During, and Right After Takeover Request." International Journal of Human–Computer Interaction (2022): 1-21.
\bibitem{human-machine_29}Politis, Ioannis, et al. "Designing autonomy in cars: A survey and two focus groups on driving habits of an inclusive user group, and group attitudes towards autonomous cars." International Conference on Applied Human Factors and Ergonomics. Springer, Cham, 2017.
\bibitem{human-machine_30}Benderius, Ola, Christian Berger, and Victor Malmsten Lundgren. "The best rated human–machine interface design for autonomous vehicles in the 2016 grand cooperative driving challenge." IEEE Transactions on intelligent transportation systems 19.4 (2017): 1302-1307.
\bibitem{human-machine_31}Bengler, Klaus, et al. "From HMI to HMIs: Towards an HMI Framework for Automated Driving." Information 11.2 (2020): 61.
\bibitem{human-machine_32}Wulf, Felix, et al. "Recommendations supporting situation awareness in partially automated driver assistance systems." IEEE Transactions on Intelligent Transportation Systems 16.4 (2014): 2290-2296.
\bibitem{human-machine_33}Richardson, Natalie Tara, et al. "Conceptual design and evaluation of a human machine interface for highly automated truck driving." 2018 IEEE intelligent vehicles symposium (IV). IEEE, 2018.
\bibitem{human-machine_34}Chen, Danjue, et al. "Towards vehicle automation: Roadway capacity formulation for traffic mixed with regular and automated vehicles." Transportation research part B: methodological 100 (2017): 196-221.
\bibitem{human-machine_35}Benderius, Ola, Christian Berger, and Victor Malmsten Lundgren. "The best rated human–machine interface design for autonomous vehicles in the 2016 grand cooperative driving challenge." IEEE Transactions on intelligent transportation systems 19.4 (2017): 1302-1307.
\bibitem{human-machine_36}Zandi, Babak, et al. "International study on the importance of communication between automated vehicles and pedestrians." Transportation research part F: traffic psychology and behaviour 74 (2020): 52-66.
\bibitem{human-machine_37}	Hu, Z., et al. "Toward human-centered automated driving: a novel spatiotemporal vision transformer-enabled head tracker. IEEE Vehi Technol Mag 2–9." (2021).
\bibitem{human-machine_38}Rahman, Md Mahmudur, et al. "How the older population perceives self-driving vehicles." Transportation research part F: traffic psychology and behaviour 65 (2019): 242-257. 
\bibitem{human-machine_39}Linkov, Václav, et al. "Human factors in the cybersecurity of autonomous vehicles: Trends in current research." Frontiers in psychology 10 (2019): 995.
\bibitem{human-machine_40}Kong, Qinglei, et al. "Blockchain-based privacy-preserving driver monitoring for maas in the vehicular iot." IEEE Transactions on Vehicular Technology 70.4 (2021): 3788-3799.
\bibitem{human-machine_41}Holstein, Tobias, Gordana Dodig-Crnkovic, and Patrizio Pelliccione. "Ethical and social aspects of self-driving cars." arXiv preprint arXiv:1802.04103 (2018).

%\end{thebibliography}

==> body/datasets.tex <==
\section{Datasets}

The publicity of various kinds of autonomous driving datasets have made a substantial contribution to the advancement in this area, especially for perception and end-end planning task. KITTI \cite{dataset_KITTI} provides multiple computer vision tasks on urban roads in Germany. Cityscapes \cite{dataset_seg_CityScape}, BDD100K \cite{BDD100K}, Mapillary Vistas \cite{dataset_seg_Mapillary_Vistas} have released a number of data with segmentation masks. A*3D\cite{A*3D} enriches the collection scenes, such as the dark night, rainy and snowy.

Some automobile manufacturers publish datasets collected by their vehicles, including H3D \cite{H3D}, A2D2 \cite{A2D2} and the Ford Dataset \cite{Ford}. For more details, please check the Table \ref{table:datasets}, which includes the whole frames, installed sensors and covering tasks for each dataset. Readers could find the corresponding data by their mission. For end-end planning, the environment is more crucial for developers, and the simulation platform such as Carla \cite{CARLA}, Vissim, PerScan, AirSim, Udacity self-driving car simulator, Apollo etc. could assist researchers to conduct the experiments on planning and control.

\input{tabels/datasets/datasets}

==> body/methodology/HDmap.tex <==
\subsection{HD map}

Maps are an integral part of modern autonomous driving. The information from the map supports many functions of autonomous driving, including self-orientation, vehicle control, motion planning, perception and systems management. Broadly speaking, a map is a representation of features of the real world and their locations as objects. It is a symbolic and abstract description of object features (such as buildings, roads and lakes) and non-object concepts (such as air pressure or temperature). The narrow definition of maps is that maps provide information about real-world features or phenomena and their position in 2D or 3D space.

The information provided by HDmap can be divided into three categories: topological information, geometric information and semantic information. Topology information contains connectivity information between geometric features, geometric information contains geometric shape mapping data of objects around vehicles, semantic information shows road speed limit, lane information and road classification, etc.

The data quality of autonomous driving maps consists of five components: 1) accuracy, 2) precision, 3) completeness, 4) consistency, and 5) timeliness. Accuracy is the difference or deviation between the actual value and the mapped value. Precision means the smallest discernible unit of a map. Completeness means the extent to which a map contains all real-world features, which is measured by omission (missing data) and redundancy (presence of too much data). Consistency also refers to the extent to which logical rules of data structure, attributes, and relationships are followed. Timeliness means the time between map creation and use.

In order to increasing data quality, Wong and Ellul\cite{HDmap_81}proposed geometry-based metrics as part of fitness assessment for 3D maps. Javanmardi et al.\cite{HDmap_79} defined four criteria to evaluate the vehicle location capability of maps, from the view of layout, feature adequacy, presentation quality and local similarity. Murphy and Pao\cite{HDmap_82} proposed a method for detecting unmapped or mismapped roads and parking lots in the context of map matching, resulting to a system that is more robust and can even correct errors in the underlying map. From a similar but alternative perspective, Yang and Huang\cite{HDmap_80} studied how to make autonomous vehicle systems more resistant to malicious attacks on their sensors.

==> body/methodology/communication.tex <==
\subsection{\textbf{Communication}}
As a powerful extension of the perception capabilities of autonomous driving and intelligent vehicles, the communication of intelligent vehicles not only involves the vehicles themselves, but also involves a variety of infrastructure and technical elements of transportation, communication, and other systems, and is a focused area for the integration and convergence of automotive, transportation, communication, information, and other industries. Vehicular communication technology originated from academic research and demonstration projects conducted in Europe and the United States at the end of the 20th century that focused on vehicle-to-vehicle (V2V) and vehicle-to-infrastructure (V2I) communications, which was known as vehicular ad-hoc network (VANET) \cite{hartenstein2008tutorial} or vehicular network at that time. With the development of the novel information and communication technologies, the connection and cooperation of all elements in transportation systems has been further strengthened to form a connected and cooperative autonomous driving, the concept of VANET was extended to the Internet of vehicles and it has gained wide attention due to its supporting role for industries such as intelligent transportation and autonomous driving.

%\cite{weiss2011v2x,abboud2016interworking}
%\cite{jiang2008ieee,chen2020vision}

With the expansion of the concept, the vehicular communication technology has evolved from the VANET that connects vehicles and infrastructure to the vehicle-to-everything (V2X) \cite{abboud2016interworking} that connects various elements of the transportation system such as vehicles, infrastructures, pedestrians and clouds. Specifically, V2X contains two types of technologies, dedicated short range communication (DSRC) standardized by IEEE and cellular V2X (C-V2X) standardized by the 3rd Generation Partnership Project (3GPP) \cite{chen2020vision}. In terms of communication methods, V2X communication can be subdivided into V2V, V2I, vehicle-to-pedestrian (V2P), and vehicle-to-cloud/network (V2C/N) communication. Therefore, vehicular networks can realize real-time and efficient information interaction among pedestrians, vehicles, infrastructures, and clouds, and support the massive data transmission of autonomous driving and intelligent vehicles.

\subsubsection{\textbf{Standardization of V2X Communication}}
To achieve efficient communication and interaction between heterogeneous vehicles, it is necessary to establish unified protocols and standards covering from the physical layer to the application layer. As mentioned above, based on different radio access technologies, there are two major types of V2X communication standards, namely DSRC and C-V2X. In this section, we briefly present the status and development of these two types of standards.

%\cite{weiss2011v2x,abboud2016interworking,kenney2011dedicated}
%\cite{eichler2007performance,survey_communication_7}

\textbf{\textit{1.1 DSRC}}: 
Strictly speaking, DSRC is a radio access technology for vehicular communication, but it is also used to broadly refer to vehicular communication based on this radio access technology. Currently, the technology is relatively mature, and several organizations for standardization, such as IEEE, Society of Automotive Engineers (SAE), and European Telecommunications Standards Institute (ETSI), have worked on DSRC-related standards \cite{abboud2016interworking}. Here we take the standard of the United States as an example to describe its standardization. In the United States, IEEE has developed the IEEE 802.11p and IEEE 1609 standards for the 5.9 GHz spectrum and formed the WAVE protocol stack \cite{uzcategui2009wave}. IEEE 802.11p is a communication protocol expanded from the IEEE 802.11 standard to support vehicular communication in a mobility environment \cite{survey_communication_7}. The IEEE 1609 protocol family is a high-level protocol for WAVE, including 1609.1, 1609.2, 1609.3, 1609.4, etc. \cite{teixeira2014vehicular,dibaei2022investigating}. Specifically, 1609.1 is a standard on resource management at the application layer of WAVE, 1609.2 defines secure message formats and their processing, 1609.3 defines routing and transport services, and 1609.4 mainly provides a communication standard for multi-channel cooperation. It is worth noting that the Federal Communications Commission (FCC) has already reallocated the 70 MHz dedicated spectrum for DSRC in 2019 and dedicated 20 MHz of that band for C-V2X technology. In 2020, the FCC added another 10 MHz to the previous proposal, formally allocating 30 MHz of spectrum to C-V2X communications and dropping support for DSRC communications \cite{fcc2020use}.

\textbf{\textit{1.2 C-V2X}}
The standardization of C-V2X technology by 3GPP can be divided into two phases, LTE-V2X and NR-V2X, which complement each other and are designed with forwarding and backward compatibility considerations \cite{gyawali2021challenges}. C-V2X mainly includes two types of communication methods, cellular mobile communication (using Uu interface) and sidelink communication (using PC5 interface) \cite{hasan2020securing}.
The standardization of LTE-V2X was initially completed in 3GPP Release 14, and its main application scenario was safety-oriented services for intelligent driving assistance. Release 15 enhanced the LTE-V2X technology and supported some enhanced applications of vehicular communication. To support the requirements of advanced V2X services and autonomous driving, 3GPP Release 16 and 17 carried out research on NR-V2X and enhanced the PC5 and Uu interfaces based on 5G NR, and the related standards are frozen now \cite{chen2020vision}.
LTE-V2X, based on 4G cellular communication, is the first C-V2X communication technology, which defines the basic architecture and technical principle of C-V2X combining cellular mobile communication and sidelink communication methods \cite{chen2016lte}.
NR-V2X, based on 5G communication, is an evolutionary version of LTE-V2X. It follows the system architecture and key technical principles of combining the Uu and PC5 interfaces defined in LTE-V2X. Meanwhile, to support a series of enhanced V2X services such as platooning, extended sensors, and remote driving for the future, NR-V2X is enhanced with novel technologies of 5G NR on the PC5 interface to provide higher data rate, low latency, and ultra reliable communication services. In terms of key technologies, NR-V2X supports unicast and multicast communication modes in addition to broadcast, and adaptive improvements have been made to resource allocation and synchronization mechanisms \cite{naik2019ieee}.

\subsubsection{\textbf{Innovative Studies of Vehicular Communication}}
Facing the stringent requirements of intelligent vehicles and autonomous driving for vehicular communication, researchers have proposed improvements and optimizations for the existing vehicular communication methods in several research directions of communication and networks \cite{ahmed2018cooperative}. In this part, we briefly present innovative studies for vehicular communication in terms of the physical layer, media access control, routing, and security.

\textbf{\textit{2.1 Physical Layer}}:
The physical layer is one of the important parts that affect the performance of vehicular communication, which enables the transmission of vehicle and traffic data through radio channels \cite{liang2017vehicular}. Currently, OFDM is the major modulation technology in vehicular communication \cite{wang2019networking}, thus many studies are devoted to optimizing orthogonal frequency division multiplexing (OFDM) parameters to ensure reliable and efficient data transmission \cite{arslan2017effects}. In addition, facing the requirement of data rate for communication in autonomous driving and intelligent vehicles, millimeter-wave communication \cite{ghafoor2020millimeter} and visible light communication (VLC) \cite{memedi2021vehicular} in the vehicular environment have become emerging research directions.

\textbf{\textit{2.2 Congestion Control}}:
Since the bandwidth of vehicular communication is limited, with large-scale deployment of vehicles, the access of massive terminals can lead to channel congestion and cause delay or even failure of data transmission \cite{paranjothi2020survey}. Congestion control avoids the congestion in the channel and improves the stability and reliability of data transmission through power-based, rate-based, hybrid, priority-based, and cross-layer approaches \cite{rashmi2021survey}.

\textbf{\textit{2.3 Resource Allocation}}:
Facing the dynamic channel access and multi-user interference caused by the high mobility of massive vehicles, vehicular communication maximizes the system performance by optimizing the allocation of resources such as channels, bandwidth, and transmit power \cite{ahmed2018cooperative}. For DSRC, various studies have proposed schemes such as medium access control (MAC) parameter allocation, channel allocation, and rate allocation \cite{noor2022survey}. For C-V2X, resources are efficiently utilized through centralized schemes based on clustering, cloud computing, non-orthogonal multiple access (NOMA) and semi-persistent scheduling, and distributed schemes based on location, sensing, and enhanced randomization \cite{le2021comprehensive}. In addition, machine learning, especially deep reinforcement learning, as a powerful analytical technique for complex problems, has become an important scheme for resource allocation and optimization \cite{nguyen2021drl}.

\textbf{\textit{2.4 Routing}}:
In vehicular communication, the range of one-hop communication between vehicles and other units (vehicles or infrastructure) is limited, so routing is needed to achieve long-distance data interaction between vehicles and vehicles or roadside infrastructures \cite{jeong2021comprehensive}. However, facing the frequently changing topology and unstable connections caused by the high-speed movement of vehicles, the traditional routing methods in wireless communication are no longer applicable \cite{ksouri2022towards,xia2021comprehensive}. Therefore, many studies have proposed enhanced routing schemes in vehicular communication to achieve efficient and stable data exchange, which include position-based, topology-based, geocast-based, broadcast-based, and cluster-based routing protocols \cite{wang2019networking,sun2021applications}. Various routing protocols improve the quality of service (QoS) of vehicular communication by optimizing the delay, distance, reliability, energy consumption, or security of routing \cite{belamri2021survey}. In addition, with the development of machine learning, learning-based routing protocols have also attracted more attention \cite{kayarga2021study}.


%\cite{sun2021applications,hasan2020securing}
%\cite{gyawali2021challenges,alladi2022comprehensive}
%\cite{sheikh2019survey,farooq2021survey,gyawali2021challenges}
%\cite{alladi2022comprehensive,dibaei2022investigating,talpur2022machine}

\textbf{\textit{2.5 Security}}: Intelligent vehicles interact with traffic systems through vehicular communication to improve driving safety and traffic efficiency \cite{hasan2020securing}. In this environment, attacks such as replay attacks, man-in-the-middle attacks, impersonation attacks, spoofing attacks, and malicious third-party attacks threaten the information security and even driving safety of vehicles \cite{gyawali2021challenges}. Therefore, facing the security requirements of vehicular communication, various studies prevent malicious attacks in terms of authentication, authorization, confidentiality, data integrity, and availability \cite{farooq2021survey,gyawali2021challenges}. In addition, machine learning-based attack detection and blockchain-based consensus and tamper-proof have become emerging research directions \cite{dibaei2022investigating,talpur2022machine}.

\subsubsection{\textbf{Future Research Directions}}
Vehicular communication realizes the connection and interaction among pedestrians, vehicles, roadside infrastructures, and cloud platforms. With the improvement of communication capability in the future, the vehicular communication system will not only complete the interaction of data but also realize the cooperation among vehicles, roadside infrastructures, and cloud platforms. The potential development directions of vehicular communication are as follows.

\textbf{\textit{3.1 Communication Technology Evolution and Performance Improvement}}:
With the evolution of C-V2X communication, the chips, modules, and terminals based on NR-V2X communication will be gradually commercialized. The application of the novel communication technology will significantly improve the communication performance of the vehicular communication system, and build a large bandwidth, high reliability, and low latency connection between the pedestrian, vehicle, infrastructure, and cloud. Relying on this high-performance communication technology, vehicular communication will no longer be limited to the basic assistant warning scenarios, but will further support the realization of various high-level cooperation and control scenarios, such as remote driving, sensor sharing, platooning, and advanced driving, and promote the intelligent transportation services to the next generation.

\textbf{\textit{3.2 From Data Interaction to Cooperative Intelligence}}:
With the performance improvement of vehicular communication and the development of sensing and computing technology, the function of vehicles and roadside infrastructures will no longer be limited to the reception and dissemination of information, but will further cooperate to complete the sensing, decision-making, and control in the complex traffic environment, thus realizing the highly cooperative operation of the vehicular communication system. In addition to the onboard sensors of intelligent vehicles, roadside infrastructure will deploy cameras, LiDARs, radars, and other devices. With the cooperative capability provided by vehicular communication, the sensing results of each intelligent terminal will be further shared, thus solving the ineffectiveness of perception by individual vehicles caused by low penetration of communication or obstacle occlusion.

\textbf{\textit{3.3 Integration of Communication and Computing}}: 
With the empowerment of vehicular communication, the connectivity and intelligence of vehicles will be further enhanced, resulting in vehicle-infrastructure-cloud connectivity and cooperation in various scenarios. The compute-intensive and latency-sensitive applications in these environments impose stringent requirements on communication rate, transmission reliability, computational real-time, and computing power scheduling. Facing these requirements, the communication and computation of the system can be integrated and resources can be scheduled and allocated cooperatively to support the development of autonomous driving.

==> body/methodology/control.tex <==

\subsection{\textbf{Control}}
Vehicle motion control is an important duty for enhanced driver assistance features. Many control tasks, such as lateral stability control and driving at the limits for accident avoidance, must be considered in the context of a highly automated vehicle. This section summarizes some of the major advancements in automated vehicle control during the previous few years. We will introduce the function of vehicle motion control, provide a comprehensive discussion on control strategies and discuss the state-of-the-art validation methods of control strategies.

\subsubsection{\textbf{Categories of Vehicle Motion Control}} 
We category the vehicle motion control into two sub parts, the longitudinal vehicle control and the lateral vehicle control.
%and the integration of lateral and longitudinal control.

\textbf{\textit{1.1 Longitudinal Vehicle Control}}: Longitudinal control manages the acceleration of the vehicle through the vehicle’s throttle and brake to keep a safe distance behind another vehicle, maintain the desirable velocity on the road and apply the brake as quickly as possible to avoid rear-end collisions in emergencies \cite{nobe2001overview, survey_control_6, smc_4, smc_6, smc_9, smc_10, smc_12, smc_24}.

%\cite{kim1996fuzzy,isermann1995nonlinear}

Longitudinal control strategies have been investigated in various scenarios, including platooning for connected autonomous vehicle (CAV) \cite{gong2016constrained, wei2017dynamic, arefizadeh2018platooning}, speed harmonization \cite{malikopoulos2018optimal, ma2016freeway}, trajectory smoothing \cite{li2018piecewise}, and speed management on signalized arterials \cite{altan2017glidepath, hao2018eco}. Local and string stability are crucial aspects of platoon longitudinal controllers. Local stability refers to a vehicle's capacity to maintain an equilibrium state under the condition of disturbance.  String stability refers to the magnitude of a disturbance that reduces or remains constant as it propagates through a platoon of vehicles. The control strategies for speed harmonization aim to determine the speed policy of the vehicles so that to prevent traffic break-downs and mitigate the loss of highway performance. The fundamental idea of trajectory smoothing is to improve traffic flow stability and efficiency through the longitudinal control strategy of CAV. On signalized arterials, speed management systems aim to adjust signal timing to reduce stops at signalized crossings while smoothing vehicle trajectories. Common longitudinal control strategies include Fuzzy logic \cite{kim1996fuzzy}, Proportional–Integral–Derivative (PID) \cite{choi1996robust}, model predictive control (MPC) \cite{zhou2019distributed}, game theory \cite{huang2019game}, sliding mode control (SMC) \cite{wu2019path}, Fuzzy inference system (FIS) \cite{mar2001anfis}, Lyapunov-based adaptive control approaches \cite{swaroop2001direct}, and AI-approaches \cite{chen2017learning}. The challenges dealing with within the design of the longitudinal control system include string-stable operation with tiny headway, execution of longitudinal split, and join manoeuvres subject to communication limitations \cite{dai2005approach, smc_25}.

%\cite{gong2016constrained, nobe2001overview}
%\cite{falcone2007predictive, kim2014model}
%\cite{tai2002experimental, guo2013adaptive, liu2021super, sun2019nested}

\textbf{\textit{1.2 Lateral Vehicle Control}}: 
Lateral vehicle control systems focus on the vehicle’s position in the lane. The major function of the lateral vehicle control system is to keep the vehicle in the current lane (lane-keeping), drive the vehicle to the adjacent lane (lane change), or avoid collisions with its preceding vehicle \cite{gong2016constrained}. The control tasks for lateral control are to minimize the lateral displacement and the angular error with regard to the reference trajectory \cite{survey_planning_4}. Various linear and nonlinear controllers have been reported in the literature to control the motion of the vehicle including Game theory-based approaches \cite{zhang2019game,yu2018human,talebpour2015modeling}, PID \cite{marino2011nested}, MPC \cite{kim2014model}, $H_\infty$ robust control \cite{ganzelmeier2001robustness, smc_26}, Lyapunov-based adaptive control approaches \cite{choi2000design, netto2004lateral}, Linear Parameter Varying Controllers \cite{huang2005ltv, baslamisli2009gain, besselmann2009autonomous}, SMC \cite{guo2013adaptive, liu2021super, sun2019nested}, Fuzzy logic \cite{guo2012design, arifin2022steering} and deep learning-based approach \cite{eraqi2017end}.

As the lateral control system can change the vehicles’ lane safely and perform evasive manoeuvres, it can offer potential benefits in reducing accidents and enhancing driving safety. However, full implementation of lateral vehicle control remains a real-world difficulty in lance changes and evasive maneuvers. For example, environmental factors such as weather conditions, road curves, and other various disturbances may affect the control performance and a proper lateral control strategy is needed.

%\textbf{Integration of Lateral and Longitudinal Control:}
%To couple characteristics between the lateral and longitudinal dynamics of intelligent vehicles in order to achieve difficult control objectives (e.g. sharp turn at high speed), the research on the design of constructing integrated control laws for lateral and longitudinal motions has attracted the researchers' attention.

%The integrated control of horizontal and lateral motions can be divided into decomposed control and centralized control. Decomposed coordinated control decouples horizontal and lateral dynamics, constructs horizontal and lateral control laws independently, and designs control logic to coordinate the horizontal and lateral dynamics at the same time. For example \cite{rajamani2000demonstration} designs an integrated control system that includes three components: lateral controller, longitudinal controller, and supervisor. The supervisor module is responsible to coordinate the lateral/longitudinal controller by monitoring the vehicle state in real-time.  The centralized coordinated control refers to obtaining the integrated control law by controlling the vehicle's lateral and longitudinal coupling dynamics model directly. \cite{bae2014integrated} presents a systematic design of the integrated control of vehicle lateral and longitudinal motions to maximize the capacity to transfer traction forces longitudinally and laterally in the most efficient way possible. The simulation results show that centralized coordinated control can remove the conventional simplifications on vehicle dynamics and deal with unmatched nonlinear vehicles and overcome the non-linear and strong coupling horizontal and vertical characteristics. However, it highly depends on high-quality hardware support.

%Compared to the independent control design (longitudinal or lateral) mentioned above, only a few such works on integrated control of horizontal and lateral motion have been reported, see game-theoretic approaches \cite{wang2015game,dreves2018generalized}, neural network \cite{naranjo2006acc+,rausch2017learning}, $H_\infty$ robust control \cite{peng2006robust}.

\subsubsection{\textbf{Control Methodology}} 
We introduce severval common methodologies in vehicle control.

\textbf{\textit{2.1 Proportional–Integral–Derivative (PID) Control}}: 
The generic applicability of the PID controller can make it outperform other control approaches to in-vehicle control for intelligent vehicles \cite{choi1996robust, connolly1999longitudinal, smc_7, smc_14, smc_15, smc_16, smc_17, smc_18, smc_19}. A nested PID steering control is developed for lateral control of autonomous vehicles in the condition of unknown route curvature \cite{yu2018human}. PID control has the advantages of simple structures, easy implementation, and no need to know the in-depth knowledge of the behavior of the system. However, PID parameters tuning is challenge and no optimal performance guaranteed. In addition, it is hard for PID controllers to be adaptive and robust to unknown and changeable external environments \cite{huang2017parameterized}.

\textbf{\textit{2.2 Game-theoretic Approaches}}: 
In game theory approaches, the vehicles are regarded as game participants and traffic rules are considered in the respective decision models. The decision models can mimic human behaviors by interacting with surrounding drivers, extract information from the interaction and generate the optimal control strategies, e.g. when and how to change the lane \cite{zhang2019game,yu2018human}. One advantage of the game-theoretical approaches is the consideration of the mutual influence of traffic participants, which can increase the reliability of decision-making. However, the dimension of the game can be highly increased by involving more participants and the high dimensionality of the coupled game system may result in high computational complexity.

\textbf{\textit{2.3 Fuzzy Logic Control}}: 
Similar to PID controller, Fuzzy logic control doesn’t require the mathematical model of the plant allowing the controller to adequately deal with nonlinear vehicle dynamics. Another benefit is their humanoid control actions because of the human-like rules. Using membership functions, the input variables are translated into linguistic variables. The controller's output is determined by fuzzy rules that take the form of "if-then" statements. \cite{cai2009intelligent} presents a neuro-fuzzy controller with the aim to regulate the speed in order to maintain a safe distance with respect to the vehicle in front. \cite{sun2019nested} designs a fuzzy feedback controller to optimize the parameters of membership functions and rules in order to track the reference trajectories under different driving conditions. However, parameter optimization is challenging and fuzzy inference rules with a lot of expert knowledge are also required for fuzzy logic control \cite{guo2012design}.

\textbf{\textit{2.4 Model Predictive Control}}: 
MPC is extremely popular for vehicle control, see longitudinal control \cite{ arefizadeh2018platooning, zhou2019distributed}, lateral control \cite{yu2018human}, and integrated control \cite{8885839}. The principle of MPC is to find a predictive motion solution over a longer horizon period by solving the problem at each sample time and applying the first sequence of actions. In this way, MPC simulates a receding horizon control and changes the solution set to remain accurate to upcoming information \cite{nobe2001overview}. \cite{kim2014model} proposes an MPC-based path tracking controller that incorporates the dynamic characteristics of the steering actuation system to ensure accurate and smooth tracking. The main advantage of MPC algorithms is their ability to consider multiple performance criteria of control efficiency, ride comfort, fuel consumption, and their constraint handling capability on vehicles’ physical limits and safety.  However, they are still inadequate for non-convex and high-complexity issues. Excessive computing difficulties may impede their real-time applications.

\textbf{\textit{2.5 Sliding Mode Control-based Approaches}}: 
SMC offers the capacity to adapt to unknown disturbances and matched uncertainties. A series of path following controllers based on SMC is proposed in \cite{wu2019path, guo2013adaptive} and simulation results show that the SMC controllers are robust to disturbances and provide a proper path tracking performance.  However, the model uncertainties and the disturbances are time-varying in the realistic scenario and the model accuracy greatly influences the control performance. The control performance may be degraded due to the modeling errors \cite{rausch2017learning}.

\textbf{\textit{2.6 Linear Parameter Varying Control}}: 
The LPV controller is a linear controller and has been designed together with predictive control for lateral control \cite{ganzelmeier2001robustness,choi2000design} and integrated system control \cite{gaspar2005design}. This method requires advanced knowledge of a plant model as well as real-time signals from all states during driving. A state observer is required because this is not provided by default.



\textbf{\textit{2.7 AI-guided Driving Policy Learning}}: 
Research on artificial intelligence algorithms is progressing rapidly because of the commonplace of big data. Compared to the traditional control systems, AI-guided vehicle systems do not require any system-level knowledge and have shown great potential to optimize nonlinear systems in complex and dynamic environments \cite{chen2017learning, dai2005approach, samak2011control}. Instead of designing explicit hand-engineered algorithms for lane detection, obstacle detection, path planning, and control law design separately, the AI-guided vehicle systems can combine all efforts within one framework and teach the system to perform well and generalize to new environments through learning \cite{nobe2001overview}. \cite{yu1995road} investigates a road-following system using reinforcement learning. The testing results show that the proposed algorithm can use previous driving experiences to learn how to drive in new environments and improve the road-following performance through online learning. \cite{wang2018reinforcement} uses Deep Q-Network (DQN) to train a vehicle agent to learn automated lane change behaviors. \cite{chae2017autonomous} presents a novel autonomous braking system that uses deep reinforcement learning to intelligently manage the vehicle's velocity when a potential collision is announced. \cite{naranjo2006acc+} investigates an end-to-end controller based on a convolutional neural network (CNN) to provide steering commands without engineering each autopilot component. The AI-guided control strategies are very powerful and their capacity to generalize over a variety of similar scenarios make them fit for minor deviations in the driving conditions \cite{samak2011control}. However, safety validation of these AI-guided systems is very challenging due to the opaque nature of the methods and there is no explanation for failure can be given\cite{smc_30}. In addition, the need for training data may hinder the research of AI-guided systems.

The classic PID and sliding mode control method may fail to adapt to complex environment and unknown disturbances. The MPC and LQR are based on precise mathematical models, the uncertain and nonlinear mathematical model of the vehicle during real-world driving may degrade the control performance, especially in extreme maneuverings. The fuzzy rules of the fuzzy logic systems are based on experience, and there are no qualitative rules to refer to, making them challenging to use in engineering applications. Due to the high dimensionality of the coupled game system, the design of game theory-based control strategies is challenging. The AI-based method requires significant amount of off-line computation and training and more study into interpretability and functional safety validation methodologies for AI-driven cars is needed\cite{smc_29}.



\subsubsection{\textbf{Validation Process}}
To verify vehicle motion control algorithms, a series of testing should be designed for control strategy validation. In terms of testing patterns, the validation type can be divided into simulation studies and experimental tests. Testing in the actual world can be costly in terms of time, labor, and money. Simulation studies, in contrast, are much less expensive, faster, more adaptable and can be used to create scenarios that are difficult to replicate in real life \cite{guo2012design, wang2018reinforcement}. Simulation has become a more dominating approach with the increased accuracy and speed of simulation tool. National instruments' LabVIEW, which is a graphical computing platform, is widely used in the simulation program for testing and measurement \cite{arifin2022steering}. To model vehicle dynamics, the commercial tools Carsim \cite{kim2014model,rausch2017learning,kim2011control} with ADAMS \cite{sun2019nested}, CARLA \cite{del2021autonomous}, PreScan \cite{chae2017autonomous} and Matlab/Simulink \cite{chebly2019coupled} have been utilized by researchers for simulating car behavior.  SCANeR Studio coupled with Matlab/Simulink is used to provide realistic driving conditions for testing of automated vehicle motion controllers \cite{chebly2019coupled}. Microscopic traffic simulation tools VISSIM 10.0 \cite{so2020automated} and AutonoVi-Sim \cite{best2018autonovi} are utilized for modelling traffic situation and implement automated vehicle control. It should be noticed that the model errors should be considered through the verification and validation process and an inaccurate model may result in infeasible evaluation performance.

Some researchers set simulation studies as a first step for performance validation and conduct experimental tests for further validation. In the literature, the experimental tests can be conducted by a small and lightweight vehicle \cite{system_2}, and an on-road vehicle \cite{peng2006robust, sun2019nested,arifin2022steering}. A small and lightweight vehicle is rugged and low-cost and can be carried by a single person for testing in various environmental conditions. In addition, the small and lightweight vehicle can travel at a high speed without the worry of injuring people and property. The main disadvantage is its small payload, which is insufficient to hold the computing power required for computing. On-road vehicles as Fig.  \ref{fig:system_fig_0} in contrast, can validate the control performance in diverse lighting and weather conditions, but the approval of testing such as ethical approval is needed.


%\begin{figure}[!tb]
%    \centering
%    \begin{minipage}{.21\textwidth}
%        \centering
%        \includegraphics[width=0.8\linewidth]{picture/methodology/control_robot.png}
%        \caption{A small and lightweight vehicle The proposed approach}
%        \label{fig:prob1_6_2}
%    \end{minipage}%
%    \begin{minipage}{0.24\textwidth}
%        \centering
%        \includegraphics[width=0.85\linewidth]{picture/methodology/control_car.png}
%        \caption{On-road test vehicle}
%        \label{fig:prob1_6_1}
%    \end{minipage}
%\end{figure}

\begin{figure}
\centering  %图片全局居中
\includegraphics[width=8.5cm]{picture/methodology/autonomous_cars.png}

\caption{The figure shows the appearance of autonomous vehicles. The left vehicle is the test autonomous platform of Xi'an Jiaotong University. The right vehicle is the autonomous mining truck at an open-pi mine in China.}
\label{fig:system_fig_0}
\end{figure}

%In terms of maneuver behaviors, the vehicle motion control strategies can be tested for lane keeping behavior and lane change behavior. Lane keeping and lane change are the two important operations that require and assess the ability and performance of vehicle motion functionalities. The goal of lane keeping is to execute automatic steering to keep the vehicle in the center of the road regardless of changes in traffic conditions. The control system for lane keeping, which involves longitudinal and lateral control, is usually designed to detect any variation between the controlled vehicle and the desirable path. For example, \cite{o1996vehicle} presents an $H_\infty$ lane keeping controller that can work for both curved and straight highways in the presence of uncertain road conditions. \cite{son2014robust} develops a state feedback controller to improve the lane keeping performance on curved roads. Lane changing is a maneuver that allows a fast car to pass a sluggish vehicle and may be seen all over the highway \cite{gaspar2005design,kim2011control,djoudi2020simulation}. Compared to the lane-keeping, lane-change is more challenging to control as its reliability highly relies on driving conditions, surrounding vehicles, traffic signals, and so on \cite{khodayari2010historical}.

%In respect of driving scenarios, the testing environment can be highways \cite{gaspar2005design,kumarawadu2006neuroadaptive}, an urban environment (e.g., local roads, and residential streets) \cite{peng2006robust,huang2017parameterized}, and other areas like parks, playgrounds, front yards, and backyards of a number of suburban homes, and heavily cluttered construction areas \cite{chae2017autonomous}.


==> body/methodology/detection_old.tex <==
\subsection{Perception}
%无人驾驶中的感知是指通过各型号传感器对车辆周围的三维环境进行定量测量，广义的感知包括车辆定位，目标检测与追踪，目标预测等子环节。在学术领域还有驾驶场景的深度补全、深度估计、光流估计、场景流估计，这些研究由室内机器人的环境感知任务发展而来，但是就当下的量产无人驾驶车辆而言少见基于上述研究的成果引入，其原因分析有二：其一，上述任务多基于视觉相机或深度相机采集的数据，但当今的无人驾驶车辆仍然以激光雷达为主要传感器。其二，上述任务不仅考虑了目标还考虑了背景，这无疑增加了计算单元的开销，这对以嵌入式设备或域控制器为处理核心的智能车辆提出了更高的挑战。因此本文没有涉及上述任务的综述，感兴趣的读者可以从这些文章找到这些领域在无人驾驶学术研究中的成果。

The perception in unmanned driving refers to the quantitative measurement of the three-dimensional environment around the vehicle by various types of sensors. The generalized perception includes vehicle positioning, target detection and tracking, target prediction and other sub-links. In the academic field, there are also driving scene depth completion, depth estimation, optical flow estimation and scene flow estimation. These studies are developed from the environment perception task of indoor robots. However, for the current mass production of unmanned vehicles, there are few results introduced based on the above research. First, most of these missions are based on data collected by vision cameras or depth cameras, but today's driverless vehicles still use lidar as their primary sensor. Second, the above tasks not only consider the target but also consider the background, which undoubtedly increases the overhead of the computing unit, which presents a higher challenge to the intelligent vehicle with embedded devices or domain controllers as the processing core. Therefore, there is no overview of the above tasks in this paper, but interested readers can find achievements in academic research in these areas

%(2)目标检测，无人驾驶中的目标检测可以分成对静态场景的检测和对动态目标的检测。对静态场景的检测包含车道线检测、可行驶区域和交通标志识别，低阶无人驾驶系统会通过上述的任务实现车道保持、变更速度等行为，高阶无人驾驶则会结合高精度地图融合其他任务进行精准地自主驾驶。对动态目标的检测包含对车辆、行人等全部交通参与者的位态检测，我们按照处理数据的不同划分成视觉检测、点云检测和融合检测。无人驾驶属于典型的3D任务，因此除某些任务无需3D检测外（例如交通标志识别），我们将主要关注3D目标检测而非2D目标检测。

\textit{A.2 Object  Detection} 

Target detection Target detection in unmanned driving can be divided into static scene detection and dynamic target detection. The detection of static scenes includes lane line detection, drivable areas and traffic sign recognition. The low-order unmanned system will realize lane keeping and speed change behaviors through the above tasks, while the high-order unmanned system will integrate other tasks with high-precision map for accurate autonomous driving. Detection of dynamic targets includes configuration detection of all traffic participants such as vehicles and pedestrians, which can be divided into visual detection, point cloud detection and fusion detection according to different data processing. Unmanned driving is a typical 3D task, so we will focus on 3D target detection rather than 2D target detection except for some tasks that do not require 3D detection (such as traffic sign recognition).

% 车道线检测方法分为两种：一种是传统算法，主要基于边缘特征或者是图像分割，通过图像预处理，特征提取等方式与卡尔曼滤波器等算法结合，在识别出车道线后采用后处理的方式形成最终的车道。然而这种传统方法易受到光照变化，行驶车辆，道路破损等干扰，导致效果欠佳。近年来，深度学习方法利用网络模型自动学习目标特征，具有较强的泛化能力，可以有效提高目标检测的准确率。得益于卷积神经网络的强大特征提取能力，性能也在不断提升。

%基于视觉的车道线检测任务一般包括三个主要流程，即图像预处理、车道检测与车道跟踪。其中预处理阶段最常见的程序包括感兴趣区域（region of interest，ROI）选择、去噪声和模糊、逆透视映射（inverse perspective mapping，IPM）、分割和边缘统计等。在完成预处理之后即可进行车道的检测，一般会先对车道的特征，比如边缘或颜色等进行提取，然后利用这些特征确定车道线的位置。在成功检测到车道线之后，可以使用跟踪算法，比如卡尔曼滤波器和粒子滤波器对车道进行细化与预测。

% 基于传统方法图像处理的车道线检测方法一般应用于结构化道路上。首先对输入图像进行感兴趣区域选择和去除无关元素，常用的处理方法是顶帽变换（Top-Hat Transform, 用于去除图像中的非车道标志。	一旦输入图像经过预处理，就可以提取车道特征，例如颜色和边缘特征，因此可以基于这些特征进行检测。Hough变换算法利用边缘像素图像，是以往研究中应用最广泛的车道检测算法之一。然而，该方法设计用于在开始时检测直线，在曲线车道检测中效率不高。通常可以基于模型拟合技术（如随机样本一致性（RANSAC））检测曲线车道。RANSAC通过递归测试模型拟合分数来拟合车道模型，以找到最佳模型参数。因此，它具有很强的处理异常特征的能力。最后，在车道成功检测后，可以使用卡尔曼滤波器或粒子滤波器等跟踪算法跟踪车道位置，以改进检测结果并以更有效的方式预测车道位置。

具体来说，Kang[Road lane segmentation using dynamic programming for active safety vehicles]使用Sobel算子检测车道边缘特征，并沿垂直方向将道路图像划分为多个子区域; Suddamalla[A novel algorithm of lane detection addressing varied scenarios of curved and dashed lanemarks]等人使用像素强度和边缘信息检测曲线和直线车道，并使用自适应阈值技术提取车道标记;



基于视觉的车道检测可以大致分为两类：基于特征的车道检测[9]−[19]


和基于模型的[20]−[29]。基于特征的方法依赖于车道标记特征的检测，如车道颜色、纹理和边缘。例如，在[9]中，使用Sobel算子检测噪声车道边缘特征，并沿垂直方向将道路图像划分为多个子区域。Suddamalla等人使用像素强度和边缘信息检测曲线和直线车道，并使用自适应阈值技术提取车道标记【10】。为了消除数字图像中的摄像机透视失真并提取真实的车道特征，可以通过透视变换有效地检测车道标线。Collado等人创建了道路图像的鸟瞰图，并提出了一种基于空间车道特征和Hough变换算法的自适应车道检测和分类方法【11】。文献[12]中使用了IPM和基于车道特征的聚类粒子滤波方法相结合的方法来估计多条车道。作者声称，如果在上下文中使用强lane模型，则鲁棒性较差，并且他们仅使用弱模型进行粒子滤波跟踪。除了使用彩色图像，还可以使用其他颜色格式的图像检测车道。颜色格式转换背后的一般思想是，黄色和白色车道标记可以在其他颜色域中更加清晰，因此对比度会增加。在[13]中，在车道假设阶段，使用扩展的边缘连接算法检测车道边缘。在车道验证步骤中，使用YUV格式的车道像素、边缘方向和车道标记宽度来选择候选的边缘链接对。在【14】中，使用无监督自适应分类器识别车道。彩色图像首先转换为HSV格式以增加对比度。然后，利用基于亮度值的阈值法对二值特征图像进行处理。虽然在某些正常情况下，颜色变换有助于车道检测，但它不稳定，处理阴影和照明变化的能力有限[4]。Borkar等人提出了一种分层方法来检测夜间车道【15】。采用时间模糊技术降低视频噪声，并基于自适应局部阈值方法生成二值图像。另一种域算法（LANA）中的车道查找表示频域中的车道特征【16】。该算法在频域中捕获车道强度和方向，并使用可变形模板检测车道标线。结果表明，LANA在各种条件下都具有较强的鲁棒性。在[17]中，介绍了一种时空车道检测算法。通过积累过去帧中的某些行像素生成一系列时空图像，并对合成图像应用Hough变换检测车道。在文献[18]中，基于车道梯度幅度特征和改进的Hough变换，设计了基于FPGA和DSP的实时车道检测系统。Ozgunalp和Dahnoun提出了一种改进的车道检测特征图[19]。首先利用边缘方向确定车道方向直方图，然后根据估计的车道方向对特征地图进行改进和移位。一般来说，基于特征的方法具有更好的计算效率，并且能够在车道标线清晰时准确检测车道。然而，由于假设了太多的约束，例如车道颜色和形状，这些方法的缺点包括与基于模型的方法相比，处理阴影和低可见性条件的鲁棒性较差
传统的基于图像处理的方法较大程度的依赖了车道线的颜色、形状等特征，这种方法在车道线被遮挡、污染的情况下鲁棒性较差。


%随着机器学习的发展，许多机器学习算法在计算机视觉任务中显示出巨大的优势，并且与传统方法相比，检测和识别性能显著提高。卷积神经网络是目标识别研究中最常用的方法之一。与传统的图像处理方法相比，通过使用卷积神经网络模型，车道线检测精度从80%左右显著提高到90%以上。卷积神经网络使用多个卷积核对输入进行特征提取。组成卷积核的每个元素都对应一个权重系数和一个偏差量（bias vector），类似于一个前馈神经网络的神经元（neuron）。卷积层内每个神经元都与前一层中位置接近的区域的多个神经元相连，区域的大小取决于卷积核的大小，被称为“感受野” 。卷积核在工作时，会有规律地扫过输入特征，在感受野内对输入特征做矩阵元素乘法求和并叠加偏差量[1]：其中， 表示第 层提取的特征图， 和 分别表示第 层特征的尺寸和通道数。 ， 和 是卷积层参数，对应卷积核大小、卷积步长（stride）和填充（padding）层数。基于机器学习的方法一般采用多层卷积网络对输入图像进行特征提取。然后将特征送入全连接网络（Fully Connected Neural Network，FCNN）得到输出。网络的输出一般有两类，一类是离散的分类结果，指示图像是否包含车道线。如果检测到车道线，则输出第二类结果，即对车道线位置和方向的连续估计。也有研究采用编码器-解码器结构实现车道线检测，此类方法将编码器提取到的特征送入由多层上采样层组成的解码器中，生成与输入相同大小的图像，输出仅包含车道线的二值图。随着生成对抗网络在计算机视觉中的应用，也有研究使用生成对抗网络进行车道线检测。生成对抗网络包含一个生成器和一个鉴别器，生成器一般采用编码器-解码器结构，鉴别器负责判断生成图像的真伪。通过引入生成对抗损失函数让生成器和鉴别器相互博弈来达到更好的检测效果。通过生成对抗网络得到的车道线一般比仅用编码器-解码器结构的网络更加精确。


\textbf{Lane detection} methods are divided into two types: one is the traditional algorithm, which is mainly based on edge features or image segmentation. Through image preprocessing, feature extraction and other methods combined with kalman filter and other algorithms, the final lane is formed by post-processing after identifying lane lines. However, this traditional method is prone to interference such as light changes, driving vehicles and road damage, resulting in poor results. In recent years, deep learning methods use network models to automatically learn target features and have strong generalization ability, which can effectively improve the accuracy of target detection. Thanks to the powerful feature extraction capability of convolutional neural network, its performance is also improving

Lane detection tasks based on vision generally include three main processes, that is, image preprocessing, lane detection and lane tracking. In the pre-processing stage, the most common programs include region of interest (ROI) selection, noise and blur removal, Inverse Perspective Mapping (IPM), segmentation and edge statistics, etc. Lane detection can be carried out after the completion of the pretreatment. Generally, features of the lane, such as edge or color, will be extracted first, and then the position of the lane line will be determined by using these features. After the lane lines are successfully detected, tracking algorithms such as Kalman filter and particle filter can be used to refine and predict the lane.

Lane line detection methods based on traditional image processing generally use edge extraction method to detect lane lines on structured roads. Firstly, the input image is selected for the region of interest and irrelevant elements are removed. The commonly used processing method is top-hat Transform, which is used to remove non-lane signs in the image. In morphology, top-hat Transform is an operation to extract small elements and details from a given image. The formula is where and respectively represent the images before and after the top hat transformation, represent the open operation, and represent the structure element of the top hat operation. The top hat transformation will remove objects larger than the structure element in the image, so as to delete non-lane signs such as turning signs and road text. After removing irrelevant elements, this method extracts the edge information of the image, and then uses Hough transform to find the straight lines in the edge graph. Hough transform is a method to find straight lines or curves in 2d pixels by using the global properties of images. The principle of Hough transform is to map the image space to the parameter space and convert the curves in the image space to the corresponding reference points in the parameter space. Its main advantage is that it is less affected by noise and curve discontinuities. After all the lines in the image are obtained, the final lane lines are obtained by clustering and denoising according to the slope and other features of the lines. The traditional image processing method relies on the color and shape of the lane lines to a large extent, and this method has poor robustness when the lane lines are blocked and polluted.


With the development of machine learning, many machine learning algorithms show great advantages in computer vision tasks, and their detection and recognition performance is significantly improved compared with traditional methods. Convolutional neural network is one of the most commonly used methods in object recognition. Compared with traditional image processing methods, the accuracy of lane line detection is improved from about 8\% to more than 90\% by using convolutional neural network model. Convolutional neural network uses multiple convolution check inputs for feature extraction. Each element of the convolution kernel corresponds to a weight coefficient and a bias vector, similar to neuron of a feedforward neural network. Each neuron in the convolution layer is connected to multiple neurons in the region with similar positions in the previous layer, and the size of the region depends on the size of the convolution kernel, known as the "receptive field". When the convolution kernel is working, it will regularly sweep the input features, multiply and sum the matrix elements of the input features in the receptive field, and add up the deviation [1] : where, represents the feature graph extracted at the first layer, and represents the size and channel number of the features at the first layer respectively. , and are convolution layer parameters, corresponding to the convolution kernel size, stride and padding layers. Multi-layer convolutional networks are generally used to extract features from input images based on machine learning. Then the features are sent into the Fully Connected Neural Network (FCNN) to get the output. The output of the network generally has two types. One is the discrete classification result, indicating whether the image contains lane lines. If lane lines are detected, the second type of result is output, which is the continuous estimation of the position and direction of lane lines. There are also studies using encoder-decoder structure to achieve lane line detection. In this method, the features extracted from the encoder are fed into a decoder composed of multiple up-sampling layers to generate images of the same size as the input, and the output contains only a binary graph of lane lines. Along with the application of generative adversarial network in computer vision, there are also researches on lane detection using generative adversarial network. The generative adversance network consists of a generator and a discriminator. The generator usually adopts encoder-decoder structure, and the discriminator is responsible for judging the authenticity of the generated image. The generator and discriminator play game with each other to achieve better detection effect by introducing generative adversarial loss function. Lane lines obtained by generating adversarial networks are generally more accurate than those obtained by encoder-decoder networks alone.


%交通标志检测与识别系统是无人驾驶系统中一个重要的组成部分,通过对道路上交通标志的准确识别,将识别结果反馈给上层行车控制策略系统,车辆根据行车策略做出相应的反应,提高道路安全性,更好地辅助无人驾驶系统。

\texbf{traffic sign detection} The traffic sign detection and recognition system is an important part of the unmanned driving system. Through the accurate identification of traffic signs on the road, the identification results will be fed back to the upper driving control strategy system, and the vehicle will respond accordingly according to the driving strategy to improve road safety and better assist the unmanned driving system.

%基于视觉的3D目标检测
\texbf{visual 3D object detection} The traffic sign detection and recognition system is an important part of the unmanned driving system. Through the accurate identification of traffic signs on the road, the identification results will be fed back to the upper driving control strategy system, and the vehicle will respond accordingly according to the driving strategy to improve road safety and better assist the unmanned driving system.

%基于激光的3D目标检测是指通过激光雷达捕获的点云数据进行目标3D属性的检测。由于点云本身包含了有效点的空间位置，如果该点位于目标表面即可以认为大致了解到了目标所在的位置信息，因此基于点云的3D目标检测相较于视觉3D检测在精度上有更好的表现。

\textbf{point cloud based object detection} Laser-based 3D target detection refers to the detection of 3D target attributes through point cloud data captured by lidar. Since point cloud itself contains the spatial position of effective points, if the point is located on the target surface, it can be considered that the location information of the target is roughly understood. Therefore, 3D target detection based on point cloud has better performance in accuracy compared with visual 3D detection.

%基于融合的3D目标检测
\textbf{visual and point cloud fusion 3D object detection} abc
 
%(3)目标追踪 目标跟踪是目标检测在时间轴上的延续，获得连续时间序列一系列的目标检测结果后，可关联不同时刻下的检测结果是否属于同一目标，并推算目标运动速度、加速度等不可直接观测的微分运动信息，甚至于预测目标未来时刻的运动状态。
(3) target tracking target tracking is a continuation of target detection on the timeline, obtain continuous time series after series of target detection results, can be associated with different times of the test results are belong to the same goal, and the estimation of target motion velocity and acceleration can not be directly observed, such as differential motion information, and even predict target motion state of the future time.

%(4)预测 目标跟踪是目标检测在时间轴上的延续，获得连续时间序列一系列的目标检测结果后，可关联不同时刻下的检测结果是否属于同一目标，并推算目标运动速度、加速度等不可直接观测的微分运动信息，甚至于预测目标未来时刻的运动状态。
(4) Prediction

==> body/methodology/human-mechine.tex <==
\subsection{Human Behaviors in Autonomous Vehicles}

Human behaviors and human factor issues are important topics for autonomous vehicles, as they determine the widespread acceptance of autonomous vehicles. Modelling and understanding human behaviors can also contribute to the establishment of mutual understanding and mutual trust between humans and vehicles. However, human is a highly complex system, and a unified human behavior modeling framework still need to be investigated further \cite{human-machine_1}. In this section, the human behavior and human factor issues will be discussed according to the level of autonomy (SAE J3016) as the differences in human behavior can be significant \cite{human-machine_2, smc_21}. 

\subsubsection{\textbf{Driver Assistance and Partial Driving Automation (L1-L2)}}
On L1 or L2 automated driving vehicles (ADVs), human drivers are still inside the vehicle control loop and suppose to drive (mental drive) even if the feet or hands are off the pedals and steering wheel. In this case, the human driver can benefit from a series of advanced driver assistance systems (ADAS) such as lane departure warning (LDW) \cite{human-machine_3}, lane departure assistant (LDA) \cite{human-machine_4}, adaptive cruise control (ACC) \cite{human-machine_5}, and lane-keeping assistance (LKA) \cite{human-machine_6}, etc. To provide accurate assistance to the human drivers, several popular research areas were developed, including fatigue (muscle/mental)/drowsiness detection \cite{human-machine_7}, driver intention inference \cite{human-machine_8}, attention \cite{human-machine_9}, workload \cite{human-machine_10}, emotion \cite{human-machine_11}, and distractions \cite{human-machine_12}. Such assistance systems usually can be separated into two fundamental groups, which are physical (physiological)-behavior and psychological behavior-based methods. 

%Specifically, physical-behaviors are usually related to vehicle interaction and control, distractions and drowsiness behaviors, etc. Common physiological signals include gaze, head, facial, body, hand, foot, speech, brain dynamics (Electroencephalogram, EEG), and neuromuscular dynamics (electromyogram, EMG) \cite{human-machine_13, human-machine_14}. These signals usually can measure the driver's physical state directly. On the other hand, driver psychological behaviors, such as attention, intention, emotion, mental distraction, mental workload, and mental fatigue, reflect the driver's mental cognitive states about the driving task, which cannot be detected and measured directly. Therefore, the most common approach for inferring cognitive driver states is using measurable physiological signals as model inputs and inferring the mental states by building a representation learning-based model \cite{human-machine_15}. 

\subsubsection{\textbf{Conditional Driving Automation (L3)}}
On L3 ADVs, a human driver can further engage in secondary tasks, and long-term monitoring is no longer required. The human driver is only required to be present and capable of taking over the control at any time, especially if an emergency occurs due to system malfunction and surrounding context uncertainty. However, one of the famous drawbacks of L3 automation is the human driver cannot guarantee to provide quality and safe take-over control especially facing the time-constrained decision-making situation \cite{human-machine_16}. Therefore, the most widely studied points for L3 regarding human factors issues are the design of take-over control algorithms, resuming control and smooth switching of the control authority \cite{human-machine_17}. 
%Both driver and vehicle are allowed to raise the take-over request. While, when the vehicle raises the take-over request to the human driver, things can be much more challenging. For instance, it was shown that drivers’ responses to the resumption of control could be less controlled and more aggressive compared to when they were in manual control \cite{human-machine_18}. Also, drivers can easily be distracted, and long-term monitoring can lead to a higher mental workload compared to manual driving \cite{human-machine_19}. They cannot guarantee that they will be able to take over the vehicle quickly and safely, especially encountering critical situations, due to the loss of situation awareness and skill degradation caused by long-term automated driving \cite{human-machine_20}. Most of these studies rely on a better understanding of human behaviors, such as driver distraction and attention recognition \cite{human-machine_21}, as well as neuromuscular dynamic modeling for alert and assistance \cite{human-machine_22}. 

\subsubsection{\textbf{High/Fully Driving Automation (L4-L5)}}
With higher-level automation, human drivers are no longer expected to maintain a proper situation awareness level in case to control the vehicle when necessary. However, complex issues can arise as well, one of which is how humans understand and partner with the autonomous system. To enable the acceptance and behavior adaptation to the higher-level ADVs, driver trust should be developed. 

Driver trust is currently a major reason for the generalization and commercialization of automated driving vehicles. As shown in \cite{human-machine_23}, human trust in the AVs largely depends on the automation's driving performance considering the safety, comfortability, predictability, and ethical response to critical situations. A recent study \cite{human-machine_24} supported that the initial introduction of self-driving cars will cause unexpected reactions and situations, which may affect the level of trust the public has in the new technique. Choi et al. surveyed 552 drivers on their attitudes toward automated driving; it was shown that trust in autonomy is the most dominant factor \cite{human-machine_25}. According to an investigation of 162 Tesla drivers on their trust in Autopilot and Summon systems \cite{human-machine_26}, it was found that high levels of initial trust in the systems could be established if an excellent introduction to the system capability is provided, and the frequency of system usage will increase over time, regardless of whether participants experienced an automation failure. 

\subsubsection{\textbf{Human-Machine-Interface (HMI)}}
The automated driving techniques make the design of HMI even more complex as the HMI system for ADVs relies on human-centered design approaches \cite{human-machine_27} to ensure safety awareness, mutual trust, pleasure, and comfort \cite{human-machine_28}. Currently, the HMI system becomes the main module that enables the collaboration between driver and vehicle. The design of the HMI system is a system engineering task \cite{human-machine_29}, and this section focuses on the introduction of in-cabin and out-cabin HMI design. 

For L4/L5, vehicle autonomy is expected to be fully responsible for the driving tasks, and the human drivers are even no longer required to maintain driving knowledge and skills. Hence, it is hard to require the human occupier to understand the context properly. Instead, only safety-related information for the vehicle behaviors and future planning has to be reported and displayed \cite{human-machine_30}. A well classification for various types of HMI on highly ADVs was proposed in \cite{human-machine_31}. Specifically, the onboard HMI system can be divided into five categories, namely, dynamic HMI, automation HMI, information HMI, vehicle HMI, and external HMI. Three recommended HMI design factors were introduced in \cite{human-machine_32}. First, a head-up display can avoid the distraction of the human driver. Second, HMI systems should assist with time-constrained maneuvers and decisions. Last, the driver monitoring system is needed to help understand the human states for high-quality visualization and explanation. An expert evaluation study for the design of HMI was discussed in \cite{human-machine_33}. According to the expert evaluation, the two most essential functions of HMI are 1) present the automation availability, navigation, and environmental information, and 2) improve the driver's attention through speech instruction, LED bar light, and seat oscillation. 

%The external HMI is designed to extend the cooperation of the ego-vehicle with multiple surrounding vehicles and to explicitly communicate the driving intentions among the multiple agents. Based on an international survey on how ADVs perform external communication and interaction with other road users, a general expectation of effective interaction and communication can be clarified \cite{human-machine_34}. Benderius et al. argued that a complex external HMI is needed for ADVs to indicate their intent \cite{human-machine_35}. Instead, they proposed a show, don’t tell principle for external HMI to explicitly demonstrate the plans with a more general-purpose light bar. When treating the interaction between different road users as a multi-agent interaction system, the mutual-understanding is critical to such a system, and the agents should explicitly communicate their intention. External HMI for ADVs is also expected to use multi-modal signals to integrate auditory, visual, and V2V communication systems for holistic HMI system design \cite{human-machine_36}. 

%\subsubsection{Conclusion and Future Works}
%In sum, the increase of vehicle autonomy for commercial passenger cars will not reduce the necessity of human behaviors and human factors issues but may increase the complexity of these problems. The responsibility of ensuring a safe, comfortable, and pleasant journey is extremely heavy for autonomous vehicles.  Future works for HMI systems on ADVs should further focus on the development of mutual understanding and mutual trust mechanisms, ensuring communication transparency and efficiency with both onboard and surrounding users. The personalized and human-centered design approach should be highlighted to guarantee the ADVs also able to understand user characteristics and personalities in case to interact with humans more effectively (especially vulnerable users \cite{human-machine_37, \cite{human-machine_38}}). Meanwhile, security \cite{human-machine_39}, privacy \cite{human-machine_40}, and ethics \cite{human-machine_41} issues are also expected to be carefully considered. 

==> body/methodology/system.tex <==

\subsection{\textbf{System Design}}
In this section, the system design of the autonomous vehicle will be described from three essential aspects of AVs, namely, the computing systems, sensor systems, and system design for various applications.

\subsubsection{\textbf{Computing System}}
The computing system plays a vital role in AVs to guarantee safety, security, energy and communication efficiency. For a typical AV which usually can be equipped with a large number of onboard sensors, including Lidar, cameras, Radar, communication module, and GPS, etc., the data generated per minute can be huge. To ensure the efficient processing and fusing of heterogeneous information, the computing system must be well designed to process the information in real-time and maintain safe autonomous driving. According to \cite{survey_8}, there are two basic types of computing architecture that are widely used in AVs, which are the modular design method and the end-to-end design method. The modular design approach decouples the functional units into separate modules which can be easier for system implementation, fault diagnosis, and module update. Based on the modular design approach, the computing architecture of AV can be separated into the following key modules (as shown in Fig. \ref{fig:system_fig_1}), including computation, communication, storage, security and privacy, and power management. While the end-to-end computing architecture is largely motivated by current artificial intelligence and mainly relay on learning-based approaches to process the sensing data and generate control output directly \cite{system_2, system_3}. Considering the modular design approach is much more widely used and mature for computing architecture design on AVs, the following parts will review the computing systems based on this branch.

\begin{figure}
\centering  %图片全局居中
\includegraphics[width=8.5cm]{picture/methodology/system.png}

\caption{Typical computing architecture for AVs\cite{survey_8, survey_system_1, survey_system_2} }
\label{fig:system_fig_1}
\end{figure}

\textbf{\textit{1.1 Computing Hardware}}: 
There is multiple powerful computing hardware to support the real-time computation capability of AVs. Typically, the Central Processing Unit (CPU), Graph Processing Unit (GPU), Field Programmable Gate Array (FPGA), Digital Signal Processor (DSP), Application Specific Processor Unit (ASIC) and its custom-developed deep learning-oriented Tensor Processing Unit (TPU) are the widely used computing hardware on AVs nowadays \cite{survey_system_2, survey_8, smc_22}. Specifically, Nvidia published the Nvidia Drive series to support AV technology with powerful GPU support \cite{system_9}. Xilinx released the Zynq UltraScale+MPSoC automotive-grade processor based on FPGA, which achieved more energy-saving performance (14 images/W) than Nvidia Tesla K40 GPU (4 images/W) \cite{system_10}. The Mobile EyeQ6 series and TPUv4 are the leading ASIC-based solution for AVs, which show significant improvement in the computation power and energy efficiency \cite{system_11}. 

\textbf{\textit{1.2 Operating System}}: 
Real-time operating system (RTOS) is key module for the computing systems on AVs which enable the resouces management and real-time perception, planning, decision-making, and control autonomously at a fast speed \cite{survey_system_2}. OS on AVs should support real-time resource allocation, networking, filing, communication, etc. Two common RTOS kernels are QNX and VxWorks \cite{system_12, system_13}. The QNX is widely used in the automotive industry that contains CPU scheduling, interprocess communication, interrupt redirection, and timer \cite{system_12}. VxWorks is a monolithic kernel and is designed for real-time embedded systems and also can be used for safety and security \cite{system_13}. It is designed with a shared memory architecture and it supports multiple architectures like Intel, POWER, and ARM. 

\textbf{\textit{1.3 Middleware}}： 
In the middle of RTOS and application layers, the middleware layer is needed to bind the multiple autonomous driving services together to manage the application communication and schedule the sensing and computing resources. In \cite{system_7}, three influential middleware architectures, namely Robot Operating System (ROS1), ROS2, and Cyber are evaluated regarding the communication latency for autonomous driving applications. The Inter-Process Communication mechanism in ROS1 provides high compatibility and extensibility \cite{system_15}. ROS2 shows efficient performance in real-time distributed systems based on the Data Distribution Service (DDS)-based communication scheme \cite{system_16}. Then, the Cyber is a recently published middleware architecture by Baidu Apollo, which is primarily designed for autonomous driving. 

\cite{system_7} summarised the three architectures based on a comparison study, it was found that 1) the communication through a shared memory mechanism is the optimal solution considering the performance and reliability of AVs; 2) Data copy and serialization/deserialization operation in the middleware layer are the main attributes of communication overhead. 3) Optimization in communication characteristics can bring significant benefits to computation efficiency. 4) the higher the performance of the platform, the more likely the communication becomes the bottleneck for processing speed. 5) Additional latency can be introduced if the publishing frequency and corresponding processing time are not well calibrated. 

In sum, middleware can be a contributor to the end-to-end latency and to avoid becoming the performance bottleneck for the overall computing system, the communication and management in the middleware should be carefully designed.

\textbf{\textit{1.4 Metrics for Computing Systems on AVs}}: 
In \cite{survey_system_1}, the authors identified seven evaluation metrics for the computing system on AV, which are accuracy, timelines, power, cost, reliability, privacy, and security. A brief summary of the characteristics of these metrics is demonstrated in Table \ref{table:system_table_1}. 

\input{tabels/methodology/system_tabel_1}

\textbf{\textit{1.5 Constraints for Computing Systems on AVs:}}
Though computing systems on AVs have achieved significant improvement in recent years, there are still several essential constraints exist which can delay the wide deployment of commercial AVs. In \cite{survey_system_1}, five major design constraints, namely, performance constraints, predictability constraints, storage constraints, thermal constraints, and power constraints for AVs are identified and analyzed. 

Specifically, performance constraints mainly exist at the application level as shown in \ref{fig:system_fig_1}. In terms of the fundamental functions of AVs, including perception, planning and decision-making, and control, the gap between machine and human performance still exists. It is stated that the frame rate and processing latency are two main performance constraints for the AVs. The human driver can react to an event with the action within 100-150ms, therefore, for safety concerns, the vehicle should react even faster than the human driver within a latency of 100ms at a frequency of at least once every 100ms as well \cite{survey_system_1}. 

Predictability is another constraint which is defined from both the temporal aspects (meet the time deadline) and functional aspects (making the correct decision). Despite the conventional mean latency metric, the tail latency (99.99th-percentile latency) should also be used to satisfy the stringent predictability requirement \cite{survey_system_1}.

The storage constraint is an essential aspect and bottleneck for energy-saving and computing performance on AVs. It is shown that one AV can generate 2 to 40 TB of data per day \cite{survey_8}. The tens of TBs of storage space per day would require high storage speed and space for the vehicle. Besides, the real-time data storage and the transfer would also require a significant boost in energy and power usage. 

The thermal constraints of the AVs can be a serious consideration as well. There are two typical aspects of the thermal constraints which are 1) the temperature to keep the computing system working at operational range, and 2) the heat generated by the computing system should lead to limited impact on the vehicle thermal profile \cite{survey_system_1}. It is shown that without the cooling system, every 1 kW power consumption by the computing system would increase the in-cabin temperature up to 10℃ per minute \cite{system_17}. Therefore, usually, the computing system should be implemented in a climate-controlled area which means an additional cooling system is needed to mitigate the thermal impact of the computing system \cite{ system_17}. 

Last, power constraint is another critical aspect which can significantly influence the capability of AV. According to \cite{survey_system_1}, the power constraint of the computing system contains three major aspects which are power consumption of the computing system, consumption of the storage, and cooling overhead. The computing consumption and additional energy consumption for storage and cooling would dramatically decrease the millage of AVs, especially the electric AVs. For instance, the miles per gallon (MPG) rate can be reduced by one for every additional 400 W energy usage, and an energy-hungry system like GPUs can reduce the fuel efficiency by up to 11.5\% \cite{survey_system_1}. Therefore, more energy-efficient computing systems and green AI techniques are extremely expected for AVs in the future. 

\subsubsection{\textbf{Sensor Systems}}
Sensor systems on AVs provide essential sensing and detection data to the computation units. Common onboard sensors for AVs include Lidar, Radar, cameras, ultrasonic, GPS, IMU, and GNSS, etc. Dues to the large uncertainty properties during driving, AVs should rely on multiple sensor fusion to guarantee driving safety. Hence, in this part, the characteristics of common sensors and sensor fusion techniques are reviewed. 

\textbf{\textit{2.1 Sensors in AVs}}: 
De Jong et al. classified the sensors on AVs into smart sensors and non-smart sensors according to the internet-of-things concept in \cite{survey_hardware_3}. Smart sensors on AVs refer to those that can provide extra detection or perception information, such as object detection/tracking, and other event description from the camera, Lidar, or Radar systems. On the contrary, non-smart sensors are those which only provide raw data for processing. The study of the characteristics of on-board sensor systems has been widely studied in \cite{survey_hardware_3, system_20, system_21, survey_12}. A brief description of the different sensors and selected review studies are shown in Table \ref{table:system_table_2}. 

\input{tabels/methodology/system_tabel_2}

%\textbf{Sensor Fusion Technologies}
%Sensor fusion technologies have been widely studied for AVs \cite{system_8, system_20}. It improves the driving safety and detection robustness by reducing the detection uncertainties, false alarm rate, and overcoming the shortcomings of the individual sensor systems \cite{system_8}. It is shown that three primary sensor fusion methods for perception-purpose can be found in the literature, which are camera-Lidar, camera-Radar, and camera-Lidar-Radar \cite{system_8}. From the architectural point of view, sensor fusion can be divided into three levels, which are low-level fusion (LLF), mid-level fusion (MLF), and high-level fusion (HLF) (as shown in \ref{fig:system_fig_1}). Regarding the LLF, raw data are normally fused at an earlier stage to reduce the noise and uncertainty in the sensing results. However, precise sensor calibration is needed when applying LLF. The MLF is also known as feature fusion. It fuses abstracted feature information such as colour, location, and motion patterns from the corresponding sensors and further performs detection and recognition based on the fused features. Last, HLF is a framework to perform high-level information or decision fusion and make final results based on the individual results like detection and tracking from the corresponding sensors. In \cite{survey_static_3}, an algorithm fusion method for perception was also discussed based on the algorithm redundancy and parallel testing consideration. In \cite{system_20}, the sensor fusion strategies are systematically classified into four categories, which are fusion based on discernible units, fusion based on complementary features, fusion based on target attributes, and fusion based on a multi-source decision.

%Regarding the sensor fusion algorithms, currently, a large number of studies are based on deep learning methods. Deep learning networks such as convolutional neural networks (CNN) and visual transformers can be used as backbone networks to process the data from different sensors, extract the temporal-spatial patterns, and share information at either early-stage, mid-stage, or late-stage \cite{system_29, system_43}. Accordingly, the end-to-end learning processing can be developed for sensor fusion without hand-craft feature engineering. Despite the deep learning-based approach, conventional methods usually focus on knowledge-based methods, statistical and probabilistic methods, etc. The most successful methods including the Kalman filter, unscented Kalman filter, and particle filter has been broadly discussed in \cite{system_44, system_45, system_46}. In sum, it is shown that DL-based sensor fusion technologies are gaining great advantages nowadays in terms of accuracy, efficiency, and generalization, therefore, it is becoming one of the hottest research topics for AVs.

\textbf{\textit{2.2 System Design for Autonomous Vehicles with Various Application Scenarios}}: 
The system design of AVs is also heavily dependent on the application scenarios, policies, and regulations. Nowadays, the most commonly used standard for autonomous vehicles regarding safety, communication, and design can be found in \cite{system_47}. The standard roadmap in \cite{system_47} covers the current and ongoing standards for safety and assurance, perception, decision-making, data, security, infrastructures, and human factors. It should also be noticed that the design of the autonomous vehicle shall consider the specific application domains as well. For example, the autonomous mining truck and its testing techniques have been summarized in \cite{system_48}, which shows significantly different considerations compared to passenger cars. Other successful applications of autonomous vehicles at airports, harbours, and for logistic purposes can be found in \cite{ system_51}. Clearly, each specific autonomous vehicle requires significantly different concerns in the overall system design and should respect the specific real-world application environment. 

Another emerging research areas for system design in AVs are the design of the explainable interface for AVs. Explanation of the perception, localization, decision-making, and control to the human occupier is an essential design requirement for future AVs to enhance the human trust and acceptance of the AVs for worldwide commercialization \cite{survey_11}. The Explainability of AVs can be further divided into interpretability and completeness. Further, interpretability has two main branches, namely, transparency and post-hoc explanation \cite{survey_explainable}. Meanwhile, local explanation and global explanation also requires different system design for the AVs \cite{survey_explainable}. In sum, the design criteria for an explainable interface of AVs will contribute to the societal and legal requirements of the AVs, and more importantly enable safer, transparent, public-approved, and environmentally friendly AVs \cite{system_54}.

==> body/methodology/testing.tex <==

\subsection{Testing}
Vehicle testing has become a popular research topic in the field of intelligent vehicles since 2016. On one hand, several companies that produce intelligent vehicles encountered vehicle accidents during testing or running, which rises urgent demand to identify causes of accidents and fix complicated intelligent vehicle systems. On the other hand, researchers are increasingly interested in intelligence testing of generalized intelligent systems.  (Artificial Intelligence Test A Case Study of Intelligent Vehicles；Parallel Testing of Vehicle Intelligence via Virtual-Real Interaction).

As the research progresses, researchers gradually build a framework of conducting research. They summarize effective methods and focused on several key works \cite{sn_1, sn_2, sn_5, testing_tiv}.


First of all, they clarified concepts of function testing, performance testing, intelligence testing and other testing concepts. In short, function testing focuses on whether vehicle or its component can obtain the required output for a specific input under given particular conditions (for example, can Lidar give output of more than 3 cloud points for a 1m*1m object located at 200m away). Performance testing focuses on whether vehicle can obtain the required output for a specific range of input under given range of conditions. Intelligence testing further requires vehicle to perform reasonable and intelligent perception, decision making and control strategy for a broader and more abstract driving scenario. (Intelligence Testing for Autonomous Vehicles A New Approach).



Secondly, for the intelligence testing of intelligent vehicle, currently most of researchers conduct analysis from the view of behavioral intelligence of artificial intelligence. They believe that if an intelligent vehicle drives successfully and smoothly under a given traffic scenario, then it is equipped with driving intelligence of such scenario. As a consequence, it is a hot research topic of how to determine the necessary scenarios for testing. Addressing this need, the International Organization for Standardization proposes an international standard for functional safety (ISO 26262) aiming to point out the functional output should vehicle obtain for a particular scenario and input. Furthermore, in order to reduce the dangers by unacceptable risks due to a lack of system estimated function (inadequate design or performance limitation) or foreseeable human error, the International Organization for Standardization proposes the estimated functional safety standard (ISO 21448) for functional testing of those functions that are affected by external environment, such as automatic emergency braking (AEB) system, lane keeping system and other advanced driving assistance systems. However, for the intelligence testing of intelligent vehicles, the necessary scenarios are numerous. So far, it is hard to efficiently and reliably test the intelligence of vehicle by the method of finding ideal relationship between input and output based on human expert specified testing scenarios. (Scenario-Based Test Automation for Highly Automated Vehicles A Review and Paving the Way for Systematic Safety Assurance).


Thirdly, considering the difficulty of constructing scenarios and the trend of data-driven machine learning modelling in most of artificial intelligence systems, researchers propose several algorithms to generate scenarios semi-automated or fully automated by learning from naturalistic driving data. Especially, researchers are strongly interested in two problems. One of the problems is how to quickly identify difficult testing scenarios, so as to avoid wasting time in simple testing scenarios which does not help improve vehicle performance. (Accelerated Evaluation of Automated Vehicles Safety in Lane-Change Scenarios Based on Importance Sampling Techniques；Testing Scenario Library Generation for Connected and Automated Vehicles, Part I: Methodology；Testing Scenario Library Generation for Connected and Automated Vehicles, Part II: Case Studies；Intelligent driving intelligence test for autonomous vehicles with naturalistic and adversarial environment). The other problem is how to cover all possible scenarios as much as possible, so as to avoid intelligent vehicle encountering untested scenarios that are hard to deal. (A Theoretical Foundation of Intelligence Testing and Its Application for Intelligent Vehicles；Heterogeneous Driver Modeling and Corner Scenarios Sampling for Automated Vehicles Testing). Apparently, it is difficult to balance those two problems, and it remains unsolved. It is helpful to reveal intelligence limitation of intelligent vehicles by finding corner cases, which is worth to be studied further. (Corner Cases for Visual Perception in Automated Driving: Some Guidance on Detection Approaches)


Lastly, as it is cost and time consuming to conduct real tests, most of researchers focuses on virtual tests based on simulation. (Creating a Digital-Vehicle Proving Ground；China 12-Year Quest of Autonomous Vehicular Intelligence The Intelligent Vehicles Future Challenge Program；Verification and Validation of Intelligent Vehicles Objectives and Efforts from China). Experience of some famous companies such as Waymore and nVidia shows that (Waymo Simulated Driving Behavior in Reconstructed Fatal Crashes within an Autonomous Vehicle Operating Domain；Towards Optimal Strategies for Training Self-Driving Perception Models in Simulation) well-designed virtual tests can effectively identify the weakness of vehicles and provide useful modification solutions. Currently, relevant researches are focused on how to ensure the intrinsic behavioral rationality and external manifestation variety of simulated object in simulation systems. For example, some researchers discuss how to mimic human driver’s behavior by learning from daily collected driving data, so that interactions between manned vehicle and unmanned vehicle can be correctly reproduced in simulation systems. (A Systematic Solution of Driving Behavior Modeling and Simulation for Automated Vehicle Studies). How to transform images by deep learning models, and obtain rarely seen special scene images from transforming daily driving collected scene images has been favored by many researchers. (Driving in the Matrix Can Virtual Worlds Replace Human-Generated Annotations for Real World Tasks；InstaFormer Instance-Aware Image-to-Image Translation with Transformer)


So far there are still many difficulties need to be solved in the field of intelligent vehicle testing. It can be forecasted that the next decade will be an important stage of further rapid development of this field.

==> body/overall.tex <==
\section{Overall}

\input{tabels/overall/survey_number}

We select $124$ \cite{survey_1, survey_2, survey_3, survey_4, survey_5, survey_6, survey_7, survey_8, survey_9, survey_10, survey_11, survey_12, survey_13, survey_loca_1, survey_loca_2, survey_loca_3, survey_loca_4, survey_loca_5, survey_loca_6, survey_loca_7, survey_loca_8, survey_loca_9, survey_loca_10, survey_loca_11, survey_loca_12, survey_loca_13, survey_loca_14, survey_loca_15, survey_loca_16, survey_loca_17, survey_static_1, survey_static_2, survey_static_3, survey_static_4, survey_static_5, survey_static_6, survey_static_7, survey_static_8, survey_static_9, survey_static_10, survey_dynamic_1, survey_dynamic_2, survey_dynamic_3, survey_dynamic_4, survey_dynamic_5, survey_dynamic_6, survey_dynamic_7, survey_dynamic_8, survey_dynamic_9, survey_dynamic_10, survey_dynamic_11, survey_dynamic_12, survey_dynamic_13, survey_dynamic_14, survey_dynamic_15, survey_dynamic_16, survey_dynamic_17, survey_dynamic_18, survey_dynamic_19, survey_dynamic_20, survey_dynamic_21, survey_dynamic_22, survey_dynamic_23, survey_dynamic_24, survey_dynamic_25, survey_dynamic_26, survey_dynamic_28, survey_scene_1, survey_scene_2, survey_scene_3, survey_tracking_1, survey_tracking_2, survey_prediction_1, survey_prediction_2, survey_planning_1, survey_planning_2, survey_planning_3, survey_planning_4, survey_planning_5, survey_planning_6, survey_e2e_1, survey_e2e_2, survey_control_1, survey_control_2, survey_control_3, survey_control_4, survey_control_5, survey_control_6, survey_control_7, survey_system_1, survey_system_2, survey_system_4, survey_system_5, survey_hardware_1, survey_hardware_2, survey_hardware_3, survey_software_1, survey_communication_1, survey_communication_2, survey_communication_3, survey_communication_4, survey_communication_5, survey_communication_6, survey_communication_7, survey_communication_8, survey_communication_9, survey_communication_10, survey_communication_11, survey_communication_12, survey_communication_13, survey_communication_14, survey_communication_15, survey_simulation_1, survey_simulation_2, survey_explainable, survey_human_machine_1, survey_special_1, survey_special_2, survey_special_3, survey_special_4, survey_special_5, survey_special_6} survey articles in our paper and the Table \ref{table:overall_number} shows the categories and the corresponding numbers of papers. All the surveys are divided into several parts, including the integral \cite{survey_1, survey_2, survey_3, survey_4, survey_5, survey_6, survey_7, survey_8, survey_9, survey_10, survey_11, survey_12, survey_13}, localization \cite{survey_loca_1, survey_loca_2, survey_loca_3, survey_loca_4, survey_loca_5, survey_loca_6, survey_loca_7, survey_loca_8, survey_loca_9, survey_loca_10, survey_loca_11, survey_loca_12, survey_loca_13, survey_loca_14, survey_loca_15, survey_loca_16, survey_loca_17}, static object detection \cite{survey_static_1, survey_static_2, survey_static_3, survey_static_4, survey_static_5, survey_static_6, survey_static_7, survey_static_8, survey_static_9, survey_static_10}, dynamic object detection \cite{survey_dynamic_1, survey_dynamic_2, survey_dynamic_3, survey_dynamic_4, survey_dynamic_5, survey_dynamic_6, survey_dynamic_7, survey_dynamic_8, survey_dynamic_9, survey_dynamic_10, survey_dynamic_11, survey_dynamic_12, survey_dynamic_13, survey_dynamic_14, survey_dynamic_15, survey_dynamic_16, survey_dynamic_17, survey_dynamic_18, survey_dynamic_19, survey_dynamic_20, survey_dynamic_21, survey_dynamic_22, survey_dynamic_23, survey_dynamic_24, survey_dynamic_25, survey_dynamic_26, survey_dynamic_28}, scene understanding \cite{survey_scene_1, survey_scene_2, survey_scene_3}, tracking \cite{survey_tracking_1, survey_tracking_2}, prediction \cite{survey_prediction_1, survey_prediction_2}, planning \cite{survey_planning_1, survey_planning_2, survey_planning_3, survey_planning_4, survey_planning_5, survey_planning_6}, E2E \cite{survey_e2e_1, survey_e2e_2}, control \cite{survey_control_1, survey_control_2, survey_control_3, survey_control_4, survey_control_5, survey_control_6, survey_control_7}, system \cite{survey_system_1, survey_system_2, survey_system_4, survey_system_5}, hardware \cite{survey_hardware_1, survey_hardware_2, survey_hardware_3}, software \cite{survey_software_1},  communication \cite{survey_communication_1, survey_communication_2, survey_communication_3, survey_communication_4, survey_communication_5, survey_communication_6, survey_communication_7, survey_communication_8, survey_communication_9, survey_communication_10, survey_communication_11, survey_communication_12, survey_communication_13, survey_communication_14, survey_communication_15}, simulation \cite{survey_simulation_1, survey_simulation_2}, explainable \cite{survey_explainable}, human-machine interaction \cite{survey_human_machine_1}, and special scenes \cite{survey_special_1, survey_special_2, survey_special_3, survey_special_4, survey_special_5, survey_special_6}. Table \ref{tabel:overall_key_surveys} presents the a few highly cited surveys of each sub-sections with more than 100 times cited which are useful for autonomous driving researchers. We provide the title of these articles with the categories, citation times, published year and some special key words which assist researchers to locate the paper quickly. We also draw a timeline and place each review article on the axis Fig. \ref{fig:whole_surveys}. Readers can clearly identify the research area and the published journal of each article according to the abbreviations, and locate the article title and other information by the cite indexes.

\input{tabels/overall/survey_top}

\begin{figure*}
\centering  %图片全局居中
\includegraphics[width=18cm]{picture/overall/surveys_years.png}

\caption{We provide all the collected papers on the time axis with abbreviations, consisting of the categories, published journals and the cite index. For example, Int${\_}$TIV[2] represents this article can be found at the reference list with index 2, and it belongs to the "Integral" category and published at IEEE Transaction on Intelligent Vehicle(TIV). Different categories are in different colors.}
\label{fig:whole_surveys}
\end{figure*}

==> body/perspectives_future.tex <==
\section{Perspectives and  Future}

\subsection{Independent Task:}

\input{body/perspectives&future/perception}

\input{body/perspectives&future/planning}

\input{body/perspectives&future/control}

\input{body/perspectives&future/testing}

\input{body/perspectives&future/interaction}

\subsection{Association Tasks:}

\subsubsection{\textbf{From Perception Data to Control}}

At present, it is difficult for end-to-end technology to be widely used in the real world, but such input-output mode is similar with the driving mode of human drivers, and as a result it could enhance the robustness of the system without any link of sub-tasks.

\subsubsection{\textbf{Human-Machine Hybrid Intelligence}}

Human should not be independent of automated systems. On the contrary, They should have been an important part of it, that is, human intelligence will interact with intelligent systems, and the system will learn and fit human driving thinking, so as to improve the reliability of the system \cite{Hybrid_1, hybrid_2}.

\subsubsection{\textbf{Parallel Theory in Autonomous Driving}}

Human drivers are mostly capable to detect important information from the surrounding environment and thus make rational decisions. However, this type of capability relies on a large amount of knowledge. The parallel approach could enrich the driving data for intelligent vehicles, as a result, to enhance the detection \& planning ability.\cite{parallel_1, parallel_2, parallel_3, parallel_4, parallel_5}

\subsubsection{\textbf{Interpretability and Credibility}}

Autonomous driving is used without the intervention of drivers, and the definition of responsibility after an accident has become a difficult problem. If the explicability and confidence of each link can be explicitly provided to researchers and investigators, it can not only improve the fitting ability of the algorithm, but also locate the problem more accurately  \cite{sn_3}.

\subsubsection{\textbf{From Scenario Engineering to Scenario Intelligence}}

Nowadays, the scenario datasets storage information with different formats and standards, and without effective indexing. Thus these datasets are sparsely annotated and difficult to reuse. The purpose of scenario intelligence is to uniform the description methods \& rules \cite{chenlong_tip, anno_1}.

\subsection{Ethics on Autonomous Driving:}

As the adoption of autonomous vehicles advances, it can be anticipated that various ethical issues will arise. Current research and discussions generally cover three aspects of ethical issues associated with AVs: 1) normative ethics, 2) environmental and public health ethics, and 3) business ethics. 

\subsubsection{\textbf{Normative Ethics}}

%\cite{e1,e2,e3,e4,e5}

The normative ethical issues centre around the moral dilemmas where an AV has to make a choice between alternatives that will inevitably result in the sacrifice of human lives \cite{e2,e3,e5}. Such moral dilemmas originated from the ‘trolley problem’ proposed early in 1960’s by Foot \cite{e6}. The trolley problem describes a hypothetical situation where a trolley is about to smash five people down the track, and a bystander is forced to make a choice between letting the trolley go ahead to kill five and diverting it to kill only one person on a different track. One example of adapting the trolley problem to the context of AV is given by Bonnefon et al. \cite{e2}, who designed several delicated accident scenarios where an AV has to make decisions between scarifying pedestrians or passengers and surveyed the choices held by a cohort of participants in the US. Results of the survey suggested that most participants wanted other people to buy AVs prioritising saving the most lives in the accidents – whether the passengers’ or the pedestrians’ depending on the scenario, but preferred to own an AV prioritizing protecting the passengers. The survey mechanism was expanded and developed to an online experimental platform known as the ‘Moral Machine Experiment’ \cite{e3} to explore the moral dilemmas faced by AVs from a global perspective. The data helped identify three strong preferences: the preference for sparing human lives, that for sparing more lives, and that for sparing young lives. It was found that some preferences varied considerably across counties and reflected underlying societal-level preferences for equity. In a separate study, Morita and Managi \cite{e5} surveyed the existence of the social dilemma in Japan and compared the results to those obtained in the US, as published in \cite{e3}. The results collected in Japan were found broadly similar to those in the US in terms that people would like others to buy AVs minimizing the number of fatalities but preferred to buy AVs protecting passengers. Of particular note is that participants in the US expressed generally stronger preferences for self-protective AVs when travelling with family over riding alone, while those in Japan did not demonstrate such inclination. This difference, argued by the authors, was due to the culture difference between the two countries. While discussions referring to the trolly problem in the context of AV moral decision-making have been comprehensive and rich, several researchers have expressed concerns that the AV moral dilemmas were overstressed. Goodall \cite{e7} argued that the trolley-problem-like dilemmas seemed to be rare in daily driving – very few people can remember a situation in which they had time to decide in which way they should crash. Cunneen et al. \cite{e8} argued that framing the ethical impact of AVs in terms of the trolley-problem-like dilemmas was misleading, while more realistic ethical framings should focus on present and near-future technologies including HMI, machine perception, data privacy etc. This attitude was shared by Lundgren \cite{e9}, who also questioned the methodologies in which the discussions on the AVs’ trolley problem were extended.

\subsubsection{\textbf{Environmental and Public Health Ethics}}

%\cite{e11,e12,e13,e14,e15}
%\cite{e14,e15}

In contrast to the divergence of opinions among researchers on the relevance of moral dilemmas to the state-of-the-art of AVs, a consensus seemed to have been achieved that the introduction of AVs will raise issues associated with environmental and public health ethics. AVs could benefit the environment by, e.g. optimising energy efficiency and emissions of individual vehicles and reducing traffic congestions caused by collisions \cite{e10}. Meanwhile, AVs could bring harms to the environment and public health as a result of their influence on people’s travel behaviour \cite{e11,e12,e13,e14}. The convenience and accessibility of AVs could unlock the additional travel demand from people who bears unnecessary travel needs (e.g. window shopping or inessential meeting) or who have difficulty in travel (e.g. the elderly and those with disabilities or medical conditions) \cite{e11}. The increased travel demand would in turn increased the vehicle-miles-travelled (VMT) \cite{e12}, and result in higher levels of noise and Electromagnetic fields (EMF), both of which contribute to adverse health effects \cite{e13}. In addition, several researchers shared the concern that the proliferation of AVs could discourage people from adopting healthier transportation activities such as walking and cycling \cite{e14}, which would be a risk factor for a host of non-communicable diseases (NCDs) including obesity and diabetes. 

\subsubsection{\textbf{Business Ethics}}

%\cite{e16,e17}

Another two heated debate topics raised by AVs are liability and privacy, both of which are primarily targeted on the AV industry and thus fall into the theme of business ethics. Unlike most conventional vehicle accidents where the driver takes primary liability for the vehicle’s fate, accidents associated with an AV could cause controversial legal issues regarding the apportion of liability among the industrial stakeholders of the AV technology along the supply chain, including manufacturer, software provider, operator etc. \cite{e16}. What could make the issues even worse is that these stakeholders might not even be able to predict the behaviour of an AV due to the inherent unpredictability of the machine-learning-based algorithms in use \cite{e18}. So far, the only two countries that have enacted laws to start to address AV liability issues are the UK and Germany, which respectively chose to take toleration-oriented and a control-oriented strategies. In conjunction, serious privacy risks could arise as the AV industry prosper – it would become increasingly uncomplicated for the industrial stakeholders to access the AV users’ personal information and track their daily lives \cite{e16,e18}. Over the past five years, most countries have developed new law to control the access to, use and sharing of personal data though they were not specific to AVs \cite{e18}.

==> body/perspectives_future/control.tex <==
\subsubsection{\textbf{Control}}

The motion control technology of intelligent vehicles has made remarkable progress.  However, due to the complex longitudinal and lateral dynamics of the vehicle, mutual coupling performance objectives, and the wide application of advanced communication technology, there are still many important and unsolved problems in the research of intelligent vehicle motion control that need to be explored and recognized. The following is a preliminary outlook on its possible development directions: 1) Coordinated control method of longitudinal and lateral motion of intelligent vehicle under random uncertainty and delay conditions. 2) Multi-performance objective global optimization technology for intelligent vehicle motion control. 3) Theory and method of intelligent vehicle cooperative control in the Internet of Vehicles environment. 4) Fault tolerant method for control systems. 5) Piratical application of control systems in real traffic environment

%\textbf{Coordinated control method of longitudinal and lateral motion of intelligent vehicle under random uncertainty and delay conditions}

%At present, the research on intelligent vehicle motion control mainly focuses on designing the lateral and longitudinal controllers separately by decoupling the lateral and longitudinal dynamics. However, only a few studies on integrated control have been reported. How to design an integrated control strategy that can be used in practical and can effectively utilize the correlation characteristics of lateral and longitudinal dynamics requires further exploration.

%\textbf{ Multi-performance objective global optimization technology for intelligent vehicle motion control}

%Future intelligent vehicles are not only reflected in intelligence but also need to be green and environmentally friendly. That is to say, the future intelligent vehicle motion control will consider multi-performance objectives including safety and comfort of autonomous driving, constraints on the driving economy, and emissions of intelligent vehicles. Therefore, it is necessary to explore the mathematical description of the driving performance of intelligent vehicles under multi-objective and multi-working conditions, study the conflict mechanism of multi-performance objectives such as intelligent safety, comfort, energy-saving, and environmental protection, and obtain the global optimization solutions with multi-performance objectives.

%\textbf{Theory and method of intelligent vehicle cooperative control in the Internet of Vehicles environment.}
%The growth of the Internet of Vehicles technology in recent years has played a significant role in advancing the practical use of intelligent vehicles. Vehicle sensing systems, advanced wireless communication technologies such as Vehicle-to-Vehicle (V2V) communication and Vehicle-to-Infrastructure (V2I), and cooperative control have the potential to provide real-time and comprehensive vehicle information and improve the driving performance of intelligent vehicles. The implementation of cooperative control of a "human-vehicle-road" system based on improved wireless communication technology, traffic participant interaction, and vehicle motion status will be a key focus of future research on intelligent vehicle motion control.

%\textbf{ Fault tolerant method for control systems}
%More research into how control systems deal with adversarial attacks such as communication failures, erroneous sensory inputs, and other hardware and software problems would help the industry progress toward more reliable and secure solutions.

%\textbf{Piratical application of control systems in real traffic environment}
%Designing autonomous vehicles that can grasp the rules of the road and the behavior of other road users will require more work. For example, the control strategies are needed to ensure that the controlled vehicle stop at stop signs and red lights, or obeys speed restrictions, or maneuvers through intersections and roundabouts with other cars.


==> body/perspectives_future/interaction.tex <==
\subsubsection{\textbf{Human Behaviors}}
The increase of vehicle autonomy for commercial passenger cars will not reduce the necessity of human behaviors and human factors issues but may increase the complexity of these problems. The responsibility of ensuring a safe, comfortable, and pleasant journey is extremely heavy for autonomous vehicles. Future works for HMI systems on ADVs should further focus on the development of mutual understanding and mutual trust mechanisms, ensuring communication transparency and efficiency with both onboard and surrounding users. The personalized and human-centered design approach should be highlighted to guarantee the ADVs also able to understand user characteristics and personalities in case to interact with humans more effectively. Meanwhile, security , privacy , and ethics issues are also expected to be carefully considered.

==> body/perspectives_future/perception.tex <==
\subsubsection{\textbf{Perception}}

Perception is the upstream aspect of autonomous driving systems, the results of which will heavily influence downstream tasks including planning and motion control. Combined with limited computational resources and time, perception models need to be accurate, robust, lightweight and fast. While some teams have achieved competitive results in academic research on perception, researchers still need to continue to drill down to full-scene coverage models that are industrially ready for mass production. We have summarised a few possible future research directions as following: 1) The early fusion strategies \& universal structure for multiple sensors. 2) Lifting the 2D to 3D space detection using effective transfer structures. 3) Making the intelligent vehicles have the capability of inference. 4) Developing the self-supervised strategies and reducing the relay on huge data. 5) Exploring the cooperative perception and making a dense connection to following tasks.

%\textbf{The early fusion strategies \& universal structure for multiple sensors} In multi-source sensor fusion theory, it is generally accepted that pre-fusion algorithms are distinguished by their accuracy and post-fusion algorithms by their convenience and robustness. While post-fusion has a longer history of development and is more productive, the development of pre-fusion hit a low point in the first few years. However, in the case of unmanned tasks with high data requirements, the loss of data information due to the use of multiple independent extractors can lead to unpredictable risks in dealing with small probability events, and with the recent advent of high performance matching algorithms and hardware, research on pre-fusion continues to advance. In addition, pre-fusion unified extractors are more friendly to multi-modal and multi-type data, and future perceptual models with an universal structure will allow any combination of different numbers and types of sensors.

%\textbf{Lifting the 2D to 3D space detection using effective transfer structures} LiDAR and cameras are two important sensors in sensing tasks, but there are significant differences in the space in which the two sensors represent data. Previous studies have either mapped the laser into columnar space for fusion or fused the images as a pseudo-point cloud and then used voxel methods, with poor performance. With the intervention of the Visual Transformer, some studies have adopted this method for spatial discrepancy fusion, with the location element being the key to resolving discrepancies. The current research is still in its infancy and more research is needed to validate it.

%\textbf{Making the intelligent vehicles have the capability of inference} Making autonomous driving vehicles capable of reasoning rather than a single sensing capability may help improve the ability of models to extract targets in obscured situations. The inference capability is derived from the driving habits of human drivers and can improve the accuracy of the perception model, reduce safety risks by being able to reason and assess hidden targets that may be risky with the help of other elements such as other targets and scenarios \cite{sn_6}.

%\textbf{Developing the self-supervised strategies and reducing the relay on huge data} The autonomous driving perception task uses a starvation model that requires constant replenishment of data, due to the large and unpredictable scenarios that can be encountered while driving. In order to enable intelligent vehicles to achieve L4 or higher driving levels, the model requires a large amount of manually annotated data, but its cost is unacceptable and thus, the unsupervised 3D object detection is necessary.

%\textbf{Exploring the cooperative perception and making a dense connection to following tasks} With the development of communication transmission technology, it is possible to interact with real-time information between multiple vehicles. The cooperative sensing of multiple vehicles can sense the environmental information ahead in advance, allowing more processing and judgment time for the vehicles. In addition the current perception task use its results as the main evaluating way to the model. However the evaluating criteria to running intelligent vehicles should depend on whether control commands delivered accurately and correct path maintained for a long time or not. So it is important to densely connect to downstream tasks.


==> body/perspectives_future/planning.tex <==
\subsubsection{\textbf{Planning}}
Trajectory planning technique alone is not the bottleneck of an autonomous driving vehicle. Despite this, the planning module deserves to consider the limitations in the upstream/downstream modules so that the entire driving performance is improved. The following few aspects are an outlook on some possible future directions: 1) Safe planning for imperfect perception data. 2) Balance of solution quality and speed. 3) Performance consistency in switching between different planners. 4) Interpretability enhancement for a learning-based planner.

%\textbf{Safe planning for imperfect perception data}
%Currently, most of the planning algorithms cannot cover all scenarios. The main reason is that it is difficult to guarantee perfect perception in complex external scenarios, the following is a preliminary vision of its possible future directions.
%2)	Precise description of a vehicle’s actual mobility.
%It can improve planning performance by the construction of a suitable vehicle's internal mobility, which will greatly facilitate closed-loop tracking of the planned trajectory.

%\textbf{Balance of solution quality and speed}
%It is worth exploring how to ensure both the trajectory quality and the algorithm's efficiency in dynamic and complex scenarios. Currently, to keep real-time performance, most algorithms choose sub-optimal solutions as the final trajectory, i.e. sacrificing quality for speed. However sub-optimal solutions somehow result in a lack of security.

%\textbf{Performance consistency in switching between different planners}
%Multiple trajectory planners are deployed on board, among which the most suitable one is used when the ego vehicle drives in a specified scenario or under a specified task. Hence, occasions exist when the autonomous vehicle has to switch from one planner to another. It deserves to enhance the trajectory planning safety and consistency during the switch process.

%\textbf{Interpretability enhancement for a learning-based planner}
%Learning-based planning methods are becoming a research hotspot. Due to the un-interpretability of neural networks, improving the planner's interpretability is the key to implementing this type of method.

==> body/perspectives_future/testing.tex <==
\subsubsection{\textbf{Testing}}

At present, the mainstream intelligent driving test is to conduct intelligent test from acting randomly. There are a few questions on testing. 1) Can we conduct intelligent test from thinking rationally? For example, if driving intelligence is defined from the perspective of brain like driving and mind control, and verification tests are carried out? 2) Can scene virtual simulation mature in a few years? 3) How to define the maturity and pass line of perceptual virtual simulation? 4) Is there a strong enough open source virtual simulation software to become the industry standard? 5) How is the consistency between virtual test and field test? 6) Is there enough case data publicly available?

==> tabels/datasets/datasets.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\caption{The datasets on the autonomous driving. Sc-Scene Classification, Od-Odometry, La-Lane Detection, Dr-Driveable Detection, 2D-2D Object Detection, 3D-3D Object Deteciton, Di-Disparity, OF-Optical Flow Estimation, SF-Scene Flow Estimation, PS-Point Segmentation, Se-Semantic Segmentation, Pa-Panoptic Segmentation, De-Depth Estimation, Tr-Tracking, Pr-Prediction, Pl-Planning, E2E-end-to-end, HD-providing the HD map.}
\begin{tabular}{lcp{0.15cm}p{0.15cm}p{0.15cm}p{0.15cm}p{0.15cm}p{0.15cm}p{0.15cm}p{0.15cm}p{0.15cm}p{0.15cm}p{0.15cm}p{0.15cm}p{0.15cm}p{0.15cm}p{0.15cm}p{0.15cm}p{0.15cm}p{0.15cm}p{0.15cm}p{0.15cm}p{0.15cm}p{0.15cm}p{0.15cm}p{0.15cm}p{0.20cm}}
\hline

\multicolumn{1}{c|}{\multirow{2}{*}{Dataset}} & \multicolumn{1}{c|}{\multirow{2}{*}{Frame}} & \multicolumn{7}{c|}{Sensors}                                  & \multicolumn{17}{c}{Task}                                                                                   \\ \cline{3-27} 
\multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{}                       & Li & Vi & Ra & GP & IM & Ca & \multicolumn{1}{c|}{Te} & Sc & Od & La & Dr & 2D & 3D & Di & OF & SF & PS & Se & Pa & De & Tr & Pr & Pl & E2E & HD\\ \hline

KITTI \cite{dataset_KITTI}                                         & 15K                                         & 1     & 2      & -     & 1   & 1   & - & -                        &     & \checkmark    &     &     & \checkmark    & \checkmark    & \checkmark   & \checkmark    & \checkmark    &        & \checkmark   & \checkmark   & \checkmark   & \checkmark   &     &     &     \\
CityScapes \cite{dataset_seg_CityScape}                                     & 25K                                         & -     & 2      & -     & 1   & 1   & - & 1                        &     &      &     &     & \checkmark    & \checkmark    &     &      &      &        & \checkmark   & \checkmark   &     &     &     &     &     \\
nuScenes \cite{nuScenes}                                     & 40K                                         & 1     & 6      & 5     & 1   & 1   & - & -                         &     &      &     &     & \checkmark    & \checkmark    &     &      &      & \checkmark      &     & \checkmark   &     & \checkmark   & \checkmark   &     &     \\
A2D2 \cite{A2D2}                                          & 12K                                         & 5     & 6      & -     & 1   & -   & - & -                       &     &      &     &     & \checkmark    & \checkmark    &     &      &      & \checkmark      & \checkmark   &     &     &     &     &     &     \\
Lyft L5 \cite{Lyft}                                      & -                                           & 3     & 7      & -     & -   & -   & -  & -                       &     &      &     &     &      & \checkmark    &     &      &      &        &     &     &     &     & \checkmark   &     &     \\
A*3D \cite{A*3D}                                        & 39K                                         & 1     & 2      & -     & -   & -   & -  & -                       &     &      &     &     & \checkmark    & \checkmark    &     &      &      &        &     &     &     &     &     &     &     \\
ApolloScape \cite{ApolloScape}                                  & 144K                                        &       &     &   &       &     &     &                          &     & \checkmark    & \checkmark   &     & \checkmark    & \checkmark    & \checkmark   &      &      & \checkmark      & \checkmark   &     & \checkmark   & \checkmark   &     & \checkmark   &     \\
BDD100K \cite{BDD100K}                                      & 100K                                        & -     & 1      & -     & 1   & 1   & - & -                        & \checkmark   &      &     & \checkmark   & \checkmark    &      &     &      &      &        & \checkmark   & \checkmark   &     & \checkmark   &     &     &     \\
H3D \cite{H3D}                                          & 27K                                         &1       & -   & -   &  1     & 1    & 1    &  -                        &     &      &     &     &      & \checkmark     &     &      &      &        &     &     &     & \checkmark    &     &     &     \\
Argoverse \cite{Argoverse}                                    & 22K                                         &2       &9    &-    &1       &-     &-     &-                          &     &      &     &     & \checkmark     &\checkmark      &\checkmark     &      &      &        &     &     & \checkmark    & \checkmark    & \checkmark    &     &   & \checkmark  \\
Mapillary Vistas \cite{dataset_seg_Mapillary_Vistas}                             & 25K   &1       &1   &-     &1       &-     &-     &-                          &     & \checkmark     &     &     & \checkmark     & \checkmark     &     &      &      & \checkmark       & \checkmark    & \checkmark    &\checkmark     &     &     &     &\checkmark      \\
Waymo Open \cite{Waymo}                                   & 200K                                        &5       &5    &-    &-       &-     &-     & -                         &     &      &     &     &\checkmark      &\checkmark      &     &      &      &\checkmark        &\checkmark     &\checkmark     &     &\checkmark     &     &     &     \\
Comma2k19 \cite{Comma2k19}                                    & 200K                                        &-       & 1  &-     & 1      &1     & 1    &    -                      &     & \checkmark   & \checkmark    &     &     &      &     &      &      &        &     &\checkmark    &     &     &     &     &     \\
Ford Dataset \cite{Ford}                                 & 200K                                        &4       &7    &-    &  1     &1     & -    &  -                        &     &\checkmark      &     &     & \checkmark     &  \checkmark    &     &      &      &        &     &     &     &     &     &     &     \\
PandaSet \cite{PandaSet}                                     & 16K                                         &2       &6    &-    &  1     &1     &     &  \checkmark                         &     &      & \checkmark     &  \checkmark    &      &      &     &      &  \checkmark     &        &     &     &     &     &     &     &     \\
ONCE \cite{ONCE}                                         & 1M                                          &1       & 7    &-   &-       &-     &-     &   -                       &     &      &     &     &  \checkmark    &\checkmark      &     &      &      &        &     &     &     &     &     &     &     \\
AutoMine \cite{AutoMine}                                     & 18K                                         &1       &2    & -   & 1      &1     &-     & -                         &     & \checkmark     &     &     & \checkmark     & \checkmark     &     &      &      &        &     &     &     &     &     &     &    
\\ \hline
\end{tabular}
\label{table:datasets}
\end{table*}

==> tabels/introduction/levels.tex <==



\begin{table}[]
\centering
\caption{The table shows the six levels of autonomous driving from SAE, and the Auto represents the autonomous driving, the third to. fifth line refers the character to control, sense the environment and response to accidents. The cases indicates the level of situations the intelligent system can tackle with.}
\begin{tabular}{ccccccc} \hline
Level & Name                          & Control & Perception & Accidents & Cases \\ \hline
L0    & Artificial            & Driver  & Driver     & Driver               & No               \\
L1    & Assistance                & Driver  & Driver     & Driver               & Part             \\
L2    & Partial      & System  & Driver     & Driver               & Part             \\
L3    & Conditional       & System  & System     & Driver               & Part             \\
L4    & High & System  & System     & System               & Part             \\
L5    & Full       & System  & System     & System               & All        
\\ \hline
\end{tabular}
\label{tab:introduction_levels}
\end{table}

==> tabels/methodology/system_tabel_1.tex <==
\begin{table}[]
\caption{Metrics for Computing Systems for AVs \cite{survey_8}}
\begin{tabular}{cm{6.7cm}}\toprule

\hline

Metric      & Description                                                                                                             \\ \hline
Accuracy    & Usually evaluate the difference between the predicted value and ground truth regarding the precision, recall, and other metrics.                                                                 \\ \hline
Timelines   & Evaluate the inference and processing speed of the computing system to ensure the computation can be finished before the deadline and minimize latency and tail latency, etc.                     \\\hline
Power       & Evaluate the power usage of the computing system and analysis its impact on the energy, mileage, and comfort issues for AVs.                                                                      \\\hline
Cost        & Mainly refer to the financial cost for the computing system toward board deployment.                                                                                                              \\\hline
Reliability & To guarantee the safety of the AVs, the worst-case execution time, interruption or emergency stop capabilities, and fault-tolerant should be considered.                                          \\\hline
Privacy     & To protect the privacy of all the road users including both in-cabin and surrounding users’ private data. Also, the acquisition, storage, and communication privacy should be further considered. \\\hline
Security    & The onboard security can be mainly divided into sensing security, communication security, data security, and control security.        
\\ \hline
\end{tabular}
\label{table:system_table_1}
\end{table}

==> tabels/methodology/system_tabel_2.tex <==
\begin{table*}[]
\caption{Comparative Study for Common Sensor Systems on Autonomous Vehicle.}
\begin{tabular}{cp{5cm}p{5cm}p{5cm}}\toprule
\hline
Sensors    & Advantages                                                                                                                                                                     & Disadvantages                                                                                                                                                                           & Review Studies                                                                                                           \\ \hline
Lidar      & \begin{tabular}[l]{@{}l@{}}1.Support high-resolution 3D point cloud\\ 2.Larger and wider sensing range\\ 3.Accurate object and distance detection\\ 4.Robust to lightning\end{tabular} & \begin{tabular}[p{5cm}]{@{}l@{}}1.High Cost\\ 2.Poor performance to harsh weather\\ 3.A large amount of data stream\end{tabular}                                      & \begin{tabular}[p{5cm}]{@{}l@{}}1.Point Cloud and networks \cite{survey_dynamic_16}\\ 2.SLAM \cite{ system_27, system_28}\\ 3.Sensor design \cite{system_24, system_25}\end{tabular} \\ \hline

Camera     & \begin{tabular}[p{5cm}]{@{}l@{}}1.Cost-effective\\ 2.Visual recognition and texture extraction\end{tabular}                                             & \begin{tabular}[p{5cm}]{@{}l@{}}1.Easily affected by lighting and weather.\end{tabular}                                                       & \begin{tabular}[p{5cm}]{@{}l@{}}1.Perception and networks \cite{survey_dynamic_21, survey_dynamic_5}\\ 2.Fusion \cite{survey_dynamic_15, survey_loca_10}\end{tabular}                         \\ \hline

Radar      & \begin{tabular}[p{5cm}]{@{}l@{}}1.Support extreme long sensing range\\ 2.Resilient to various environmental conditions\end{tabular}                                          & \begin{tabular}[p{5cm}]{@{}l@{}}1.Smaller data size \\ 2.Indistinguishable from static targets\end{tabular} & \begin{tabular}[p{5cm}]{@{}l@{}}1.Detection and perception \cite{survey_hardware_2, survey_dynamic_28}\\ 2.Radar Communication \cite{system_35, system_36, system_37}\end{tabular}           \\ \hline

GPS        & \begin{tabular}[p{5cm}]{@{}l@{}}1.Low cost and stable\\ 2.Non-accumulation error for GPS\end{tabular}                                                                                   & \begin{tabular}[p{5cm}]{@{}l@{}}1.Relative low accuracy for GPS and IMU\\ 2.Slow update frequency \\3. Requiring an unobstructed view\end{tabular}                                      & \begin{tabular}[p{5cm}]{@{}c@{}}1.Localization \& navigation \cite{system_38, system_39}\end{tabular}                                                                   \\ \hline

Ultrasound & \begin{tabular}[p{5cm}]{@{}l@{}}1.Low cost\\ 2.High accuracy for close range\\ 3.Resilient to adverse weather conditions\end{tabular}            & \begin{tabular}[p{5cm}]{@{}l@{}}1.Short-range detection\\ 2.Inapplicable for high speed\end{tabular}  & \begin{tabular}[p{5cm}]{@{}l@{}}1.A systematic review \cite{system_40}\\ 2.All-weather conditions \cite{system_41}\end{tabular} 
\\ \hline
\end{tabular}
\label{table:system_table_2}
\end{table*}

==> tabels/methodology/understanding.tex <==
\begin{table}[]
\caption{\textcolor[rgb]{1,0,0}{Localization methodology with advantages and limitations}}

\begin{tabular}{cll}
\hline
Method        & Advantages & Limitations                                                                                       \\\hline
GNSS & \begin{tabular}[c]{@{}l@{}}1.All-weather\\2.Easy configuration\\3.Non external sensors \end{tabular}           &\begin{tabular}[c]{@{}l@{}}1.Site requirements  \\2.GPS update frequency \\3.High-cost (high accuracy) \end{tabular}                                    \\\hline
Visual & \begin{tabular}[c]{@{}l@{}}1.Economy\\2.Rich semantic info \end{tabular}                               &\begin{tabular}[c]{@{}l@{}}1.Lightness effect \\2.Similar feature \\3.Low accuracy \end{tabular}                                                                     \\\hline
LiDAR    & \begin{tabular}[c]{@{}l@{}}1.High accuracy. \\2.Dense map\end{tabular}                 & \begin{tabular}[c]{@{}l@{}}1.Non semantic info\\2.Environmental disturbance \\3.High-cost\end{tabular}  \\\hline
Fusion            & \begin{tabular}[c]{@{}l@{}}1.High accuracy\\2.Robustness\end{tabular}                                    & \begin{tabular}[c]{@{}l@{}}1.Complexity\\2.Calibration\\3.Synchronization\end{tabular}           \\\hline
\end{tabular}         
\label{table:control_table_1}
\end{table}

==> tabels/overall/survey_number.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\centering
\caption{The table shows the categories and the number of our collected surveys.}
\begin{tabular}{llc}
\hline
\multicolumn{1}{c}{Article Categories}        & \multicolumn{1}{c}{Sub-categories}                     & \multicolumn{1}{c}{Number} \\ \hline
Integral                    & Integral                         & 13     \\
Perception & Localization              & 17     \\
Perception & Detection \& Segmentation & 45     \\ 
Planning  & Planning                  & 6      \\
Planning  & Decision-making \& E2E    & 2      \\ 
Control                    & Control                         & 7      \\ 
System     & System \& Plantform       & 5      \\
System     & Software                  & 1      \\
System     & Hardware                  & 3      \\ 
Communication               & Communication                         & 15     \\ 
Testing    & Simulation                & 2      \\
Testing    & Explanabel                & 1      \\ 
Interaction                 & Interaction                        & 1     
\\ \hline
\end{tabular}
\label{table:overall_number}
\end{table}

==> tabels/overall/survey_top.tex <==
\begin{sidewaystable*}[]
\centering
\caption{The crucial reviews and relative in formations of each sub-task on autonomous driving}
\begin{tabular}{p{13.5cm}cccc} \hline
\multicolumn{1}{c}{Article Name}                                                                                            & Category          & Cite & Year & Charectoristic \\ \hline
A Survey of Deep Learning Techniques for Autonomous Driving \cite{survey_6}                                                                 & Integral          & \textbf{509}  & 2020 & modular pipeline                \\
A Survey of Autonomous Driving: Common Practices and Emerging Technologies \cite{survey_5}                                                  & Integral                  & 485  & 2020 &  automated driving systems              \\
Self-driving cars: A survey \cite{survey_12}                                                                                           &   Integral                & 395  & 2021 &  architecture      \\
Autonomous Cars: Research Results, Issues, and Future Challenges \cite{survey_3}                                                            &   Integral                & 291  & 2019 & challenge               \\
Artificial Intelligence Applications in the Development of Autonomous Vehicles: A Survey \cite{survey_10}                                   &    Integral               & 107  & 2020 &  emerging technologies               \\
Simultaneous localization and mapping: A survey of current trends in autonomous driving \cite{survey_loca_1}                                    &    Localization               & \textbf{489}  & 2017 &   SLAM     \\
A survey of the state-of-the-art localization techniques and their potentials for autonomous vehicle applications \cite{survey_loca_2}                                 &    Localization               & 433  & 2018 & Internet of Vehicles               \\
A review of visual-LiDAR fusion based simultaneous localization and mapping \cite{survey_loca_10}                                &    Localization               & 120  & 2020 & autonomous navigation               \\
Vehicle dynamic state estimation: state of the art schemes and perspectives \cite{survey_loca_4}                                &    Localization               & 100  & 2018 & pose estimation            \\
A review of recent advances in lane detection and departure warning system \cite{survey_static_2}                                                 & Static Detection  & \textbf{185}  & 2018 & lane departure warning    \\
Advances in Vision-Based Lane Detection: Algorithms, Integration, Assessment, and Perspectives on ACP-Based Parallel Vision \cite{survey_static_3} &  Static Detection                 & 104  & 2018 & ACP parallel theory \\
Computer Vision for Autonomous Vehicles: Problems, Datasets and State of the Art \cite{survey_dynamic_13}                                            & Dynamic Detection & \textbf{532}  & 2020 &   datasets              \\
Autonomous vehicle perception: The technology of today and tomorrow \cite{survey_dynamic_5}                                       & Dynamic Detection                  & 381  & 2018 &   autonomous vehicle application  \\
Deep Multi-Modal Object Detection and Semantic Segmentation for Autonomous Driving: Datasets, Methods, and Challenges \cite{survey_dynamic_20}       &  Dynamic Detection                 & 331  & 2021 &  fusion              \\
A Survey on 3D Object Detection Methods for Autonomous Driving Applications \cite{survey_dynamic_7}                                                &  Dynamic Detection                 & 230  & 2019 & 3D object detection         \\
Benchmarking Robustness in Object Detection: Autonomous Driving when Winter is Coming \cite{survey_dynamic_8}                                       &   Dynamic Detection                & 150  & 2019 & benchmark datasets      \\
Object recognition and detection with deep learning for autonomous driving applications \cite{survey_dynamic_1}                                     &   Dynamic Detection                & 112  & 2017 & CNN and SVM      
       \\
Deep Learning-based Vehicle Behaviour Prediction For Autonomous Driving Applications: A Review \cite{survey_prediction_2}                                   &   Prediction                & \textbf{141}  & 2020 & Deep Learning      
       \\
A Literature Review on the Prediction of Pedestrian Behavior in Urban Scenarios \cite{survey_prediction_1}                                  &   Prediction                & 106  & 2018 &  Pedestrian Behavior     
       \\
A survey of motion planning and control techniques for self-driving urban vehicles \cite{survey_planning_1}                                   &  Planning                 & \textbf{1637}  & 2016 & information sharing and coordination
       \\
Planning and Decision-Making for Autonomous Vehicles \cite{survey_planning_2}                                   &  Planning                 & 561  & 2018 & fleet management
       \\
A Review of Motion Planning for Highway Autonomous Driving \cite{survey_planning_4}                                  &  Planning                 & 170  & 2020 &  Highway
       \\
Trajectory planning and tracking for autonomous overtaking: State-of-the-art and future prospects \cite{survey_planning_3}                                 &  Planning                 & 143  & 2018 &  high-speed driving 
       \\
Deep Reinforcement Learning for Autonomous Driving: A Survey \cite{survey_e2e_1}                                &  Reinforcement                 & \textbf{143}  & 2018 & Reinforcement Learning
       \\
Driving Style Recognition for Intelligent Vehicle Control and Advanced Driver Assistance: A Survey \cite{survey_control_1}                               &  Control                 & \textbf{372}  & 2017 & driving style
       \\
A Survey of Deep Learning Applications to Autonomous Vehicle Control \cite{survey_control_6}                              &  Control                 & 211  & 2021 & vehicle control
       \\
Automated guided vehicle systems, state-of-the-art control algorithms and techniques \cite{survey_control_2}                             &  Control                 & 109  & 2019 & Automated guided vehicle system
       \\
The architectural implications of autonomous driving: Constraints and acceleration \cite{survey_system_1}                       &  System                 & \textbf{290}  & 2018 &  Hardware
       \\
Edge computing for autonomous driving: Opportunities and challenges \cite{survey_system_2}              &  System                 & 235  & 2019 & Connected  
       \\
Sensor technology in autonomous vehicles: A review                           &  System \cite{survey_hardware_1}                & 108  & 2018 & Sensor Fusion
       \\
Control of connected and automated vehicles: State of the art and future challenges \cite{survey_communication_4}                       &  Communication                 & \textbf{322}  & 2018 & energy efficiency
       \\
A Survey of the Connected Vehicle Landscape—Architectures, Enabling Technologies, Applications,and Development Areas \cite{survey_communication_3}                        &  Communication                 & 283  & 2017 & vehicle-to-everything
       \\
A Survey of Vehicle to Everything (V2X) Testing \cite{survey_communication_10}                        &  Communication                 & 167  & 2019 &  V2X application
       \\
A Survey of Intrusion Detection for In-Vehicle Networks \cite{survey_communication_11}                    &  Communication                 & 133  & 2019 & Controller area network
       \\
Autonomous vehicles that interact with pedestrians: A survey of theory and practice \cite{survey_human_machine_1}                    &  Interaction                 & \textbf{378}  & 2019 &  pedestrian behavior
       \\
Collaborative vehicle routing: a survey \cite{survey_special_2}               &  Interaction                 & 213  & 2017 & transportation
\\
\hline
\end{tabular}
\label{tabel:overall_key_surveys}
\end{sidewaystable*}
